FSW-GNN: A Bi-Lipschitz WL-Equivalent Graph Neural Network

Famously, the ability of Message Passing Neural Networks (MPNN) to distinguish between graphs is limited to graphs separable by the Weisfeiler-Lemann (WL) graph isomorphism test, and the strongest MPNNs, in terms of separation power, are WL-equivalent. However, it was demonstrated that the quality of separation provided by standard WL-equivalent MPNN can be very low, resulting in WL-separable graphs being mapped to very similar, hardly distinguishable outputs. This phenomenon can be explained by the recent observation that standard MPNNs are not lower-Lipschitz. This paper addresses this issue by introducing FSW-GNN, the first MPNN that is fully bi-Lipschitz with respect to standard WL-equivalent graph metrics. Empirically, we show that our MPNN is competitive with standard MPNNs for several graph learning tasks and is far more accurate in long-range tasks, due to its ability to avoid oversmoothing and oversquashing. Our code is available at https://github.com/yonatansverdlov/Over-squashing.

==> base/packages.tex <==
% Neat and Flexible LaTeX Template
% Written by Tal Amir 2024
% https://tal-amir.github.io/
%
% File: base/packages.tex
% to be loaded from base/base.tex
%
% This file is for loading packages and setting settings related to those packages.
% Math-related macros are loaded from base/math.tex

\usepackage{appendix}

\usepackage{amsmath}
%\RequirePackage[utf8]{inputenc} % allow utf-8 input
\RequirePackage[T3,T1]{fontenc}  % load T1 and T3 font encodings
%\RequirePackage{hyperref}        % hyperlinks
\RequirePackage{url}             % simple URL typesetting
%\RequirePackage{amsfonts}       % blackboard math symbols
\RequirePackage{nicefrac}        % compact symbols for 1/2, etc.
%\RequirePackage{microtype}      % microtypography
\RequirePackage{xcolor}
%\RequirePackage{color}
%\RequirePackage{colortbl}       % used for \cellcolor
\RequirePackage{float}
%\RequirePackage{floatrow}        % for \floatfoot. does not work with the float package
\RequirePackage{nicematrix}      % For the NiceTabular table environment
\RequirePackage{booktabs}        % professional-quality tables
\RequirePackage{multirow}        % gives better control over vertical alignment than \Block[c]{2-1}{xxx}
\RequirePackage{wrapfig}
%\RequirePackage{subcaption}     % allows adding captions to subfigures
\RequirePackage{graphicx}
\RequirePackage{caption}
%\RequirePackage{enumerate}      % for roman numerals
\usepackage{subcaption}  % Required for the subfigure environment
\RequirePackage{extarrows}
\RequirePackage{etoolbox}
\RequirePackage{ifthen}         % provides \ifthenelse
\usepackage{url}
%\usepackage[normalem]{ulem}     % \sout - strikethrough font 
\usepackage{adjustbox}
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{array}
\usepackage{booktabs}

%  ----------------------- 
% ---- siunitx package ----
%  ----------------------- 
% Enables controlling the appearance of captions
%\RequirePackage{caption}
%\RequirePackage[font=small,labelfont=bf]{caption} % Make caption font size small
%\captionsetup{font=small}
%\captionsetup[table]{skip=10pt}


%  ----------------------- 
% --- pgfplots and tikz ---
%  ----------------------- 
\RequirePackage{pgfplots}
\pgfplotsset{width=6cm,compat=newest,table/search path={csv/}} 


\usepgfplotslibrary{groupplots}
\usetikzlibrary{pgfplots.groupplots}

% Externalize the figures, i.e. save them to separate PDFs
%\usepgfplotslibrary{external}
% Tal: This command tells Tikz to generate external PDF files with the plots.
% It produces an error when compiling with Texlive 2020 or through Arxiv's webpage. 
% In those cases it can simply be turned off, resulting in a slower compilation.
%\tikzexternalize


%  ---------------------- 
% --- cleveref package ---
%  ---------------------- 
%\RequirePackage{cleveref}
%\RequirePackage{cleveref} % These options might clash with the options defined in the conference style file

% Remove the word 'equation' from references:
%\crefname{equation}{}{}
%\crefrangeformat{equation}{(#3#1#4)\,--\,(#5#2#6)} % Use en-dash instead of 'to' in equation range.

% A lower-level way to remove the word 'equation' from references:
%\crefformat{equation}{(#2#1#3)}
%\crefrangeformat{equation}{(#3#1#4) to~(#5#2#6)}
%\crefmultiformat{equation} {(#2#1#3)} { and~(#2#1#3)} {, (#2#1#3)} { and~(#2#1#3)}


%  --------------------- 
% --- siunitx package ---
%  --------------------- 
\RequirePackage{siunitx} % for displaying percents and other units
\sisetup{detect-all, group-separator = {,}, output-decimal-marker={.}}
%\sisetup{detect-weight=true,detect-inline-weight=math}
\DeclareSIUnit{\million}{\textup{million}}
\DeclareSIUnit{\millisecond}{\milli\second} 



==> figures/fig_dirichlet_newer.tex <==
\begin{figure}[t]
    \input{tikz_dirichlet.tex}
    \caption{MAD Energy vs. Number of MPNN layers for various models on the Ring long-range task}
    \label{fig:oversmoothing}
\end{figure}

==> icml_addition_after_begin_document.tex <==
\twocolumn[
\icmltitle{\TheDocumentTitle}

% It is OKAY to include author information, even for blind
% submissions: the style file will automatically remove it for you
% unless you've provided the [accepted] option to the icml2025
% package.

% List of affiliations: The first argument should be a (short)
% identifier you will use later to specify author affiliations
% Academic affiliations should list Department, University, City, Region, Country
% Industry affiliations should list Company, City, Region, Country

% You can specify symbols, otherwise they are numbered in order.
% Ideally, you should not use this facility. Affiliations will be numbered
% in order of appearance and this is the preferred way.
\icmlsetsymbol{equal}{*}

\begin{icmlauthorlist}
\icmlauthor{Yonatan Sverdlov}{mathfaculty}
\icmlauthor{Yair Davidson}{mathfaculty}
\icmlauthor{Nadav Dym}{mathfaculty,csfaculty}
\icmlauthor{Tal Amir}{mathfaculty}
\end{icmlauthorlist}

\icmlaffiliation{mathfaculty}{Faculty of Mathematics, 
Technion–Israel Institute of Technology,
Haifa, Israel.}

\icmlaffiliation{csfaculty}{Faculty of Computer Science, 
Technion–Israel Institute of Technology,
Haifa, Israel}

\icmlcorrespondingauthor{Tal Amir}{talamir@technion.ac.il}
\icmlcorrespondingauthor{Nadav Dym}{nadavdym@technion.ac.il}

% You may provide any keywords that you
% find helpful for describing your paper; these are used to populate
% the "keywords" metadata in the PDF but will not be shown in the document
\icmlkeywords{Machine Learning, ICML}

\vskip 0.3in
]

% this must go after the closing bracket ] following \twocolumn[ ...

% This command actually creates the footnote in the first column
% listing the affiliations and the copyright notice.
% The command takes one argument, which is text to display at the start of the footnote.
% The \icmlEqualContribution command is standard text for equal contribution.
% Remove it (just {}) if you do not need this facility.

\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
%\printAffiliationsAndNotice{\icmlEqualContribution} % otherwise use the standard text.


==> latexmkrc <==
# This is the configuration for latexmk
# Enabling write18 and shell escape for pdflatex
# This is probably needed for \tikzexternalize, not sure
$pdflatex = 'pdflatex --enable-write18 --shell-escape %O %S';


==> tables/table_empirical_distortion.tex <==
\newcommand{\oomcell}{{{\begingroup{\emph{OOM}}\endgroup}}}
\newcommand{\fixheaderheight}[1]{\raisebox{-0.6ex}{{#1}}}

\begin{table}[htb]
\caption{\label{table_empirical_distortion}Empirical distortion evaluation}\label{tab:empirical_distortion}
    %
    \begingroup
    % Setting the \arraystretch above 1 increases the space between cells.
    % Using \begingroup and \endgroup makes sure that the redefinition
    % of \arraystretch is only local to this table.
    { \fontsize{7}{7.5}\selectfont
    \renewcommand*{\arraystretch}{0.95}
    \begin{NiceTabular}{ccccS[table-format=2.2]S[table-format=2.2]S[table-format=2.2]S[table-format=2.2]}
        \toprule % \Block[c]{1-1}{Dataset}
        \multirow{2}{*}{\fixheaderheight{Dataset}} & \multirow{2}{*}{\fixheaderheight{$d$}} & \multirow{2}{*}{\fixheaderheight{$n$}} & \multirow{2}{*}{\fixheaderheight{Method}} & \Block{1-4}{$m$} & & &    
    \\ \cmidrule(l{2pt}r{2pt}){5-8} & & & & \Block[c]{1-1}{10} & \Block[c]{1-1}{50} & \Block[c]{1-1}{200} & \Block[c]{1-1}{1000}
    %
    \\ \cmidrule(l{2pt}r{2pt}){1-8} 
    %
    \multirow{2}{*}{ModelNet} & \multirow{2}{*}{$3$} & \multirow{2}{*}{$2047$} & PSWE & 16.45 & 30.26 & \oomcell & \oomcell
    \\ & & & FSW & 2.47 & 1.46 & 1.2 & 1.08
    %
    \\ \cmidrule(l{2pt}r{2pt}){1-8} \multirow{2}{*}{Uniform} & \multirow{2}{*}{$3$} & \multirow{2}{*}{$20$} & PSWE & 10.03 & 4.5 & 3.55 & \oomcell
    \\ & & & FSW & 2.23 & 1.36 & 1.16 & 1.07
    %
    \\ \cmidrule(l{2pt}r{2pt}){1-8} \multirow{2}{*}{Uniform} & \multirow{2}{*}{$10$} & \multirow{2}{*}{$20$} & PSWE & 8.15 & 2.84 & 1.97 & \oomcell
    \\ & & & FSW & 2.29 & 1.41 & 1.18 & 1.08
    %
    \\ \cmidrule(l{2pt}r{2pt}){1-8} \multirow{2}{*}{Uniform} & \multirow{2}{*}{$100$} & \multirow{2}{*}{$20$} & PSWE & 7.88 & 2.74 & 1.62 & \oomcell
    \\ & & & FSW & 2.43 & 1.44 & 1.19 & 1.08
    %
    \\ \cmidrule(l{2pt}r{2pt}){1-8} \multirow{2}{*}{Uniform} & \multirow{2}{*}{$1000$} & \multirow{2}{*}{$20$} & PSWE & 7.97 & 2.7 & 1.66 & \oomcell
    \\ & & & FSW & 2.4 & 1.43 & 1.19 & 1.08
    %
    \\ \bottomrule
    \end{NiceTabular} }
    \endgroup
    %
    % \floatfoot{\parbox{1\textwidth}{\small
    %     Empirical distortion w.r.t. the Sliced Wasserstein distance of the FSW and PSWE embeddings, evaluated on real and synthetic data. Each trial considered 6000 point clouds; the numbers show the average over 200 independent trials. $d$, $n$: ambient dimension and number of points in each cloud; $m$: embedding dimension. OOM: Out of Memory---the method failed due to insufficient memory.
    % }}
    %
    {\small
        Empirical distortion w.r.t. the Sliced Wasserstein distance of the FSW and PSWE embeddings, evaluated on real and synthetic data. Each trial considered 6000 point clouds; the numbers show the average over 200 independent trials. $d$, $n$: ambient dimension and number of points in each cloud; $m$: embedding dimension. OOM: Out of Memory---the method failed due to insufficient memory.
    }
\end{table}


==> tables/table_lrgb.tex <==
\begin{table*}[ht]
    \caption{LRGB results. Best in \textbf{ bold}. Second best in \underline{underline}.}
    \label{tab:lrgb_datasets}
    %
    \centering
    \begin{tabular}{lcc}
        \toprule
        Dataset & peptides-func (AP$\uparrow$) & peptides-struct (MAE$\downarrow$) \\ \hline
        GINE \cite{Hu*2020Strategies} & 0.6621$\pm$0.0067 & \underline{0.2473$\pm$0.0017} \\
        GCN \cite{kipf2017semisupervised} & 0.6860$\pm$0.0050 & \textbf{0.2460$\pm$0.0007} \\
        GatedGCN \cite{bresson2018residual} & 0.6765$\pm$0.0047 & 0.2477$\pm$0.0009 \\
        SortMPNN \cite{davidson2024h} & \textbf{0.6914$\pm$0.0056} & 0.2494$\pm$0.0021 \\
        FSW-GNN  & \underline{0.6864$\pm$0.0048} & 0.2489$\pm$0.00155 \\ \hline
        SOTA & \textbf{0.73} & \textbf{0.242} \\ \hline
    \end{tabular}
\end{table*}


==> tables/table_mutag_protein_old.tex <==
\begin{table}[H]
\caption{Performance of different models on the MUTAG and Protein dataset.}
\label{tab:mutag}
\centering
\footnotesize
\setlength{\tabcolsep}{5pt} % Adjust column spacing
\renewcommand{\arraystretch}{0.95} % Adjust row spacing     
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Model}                & \textbf{MUTAG}        & \textbf{Protein} \\ \midrule
GIN {\scriptsize\citep{gin}}         & $89.4 \pm 5.6$        & $76.2 \pm 2.8$ \\
GCN {\scriptsize\citep{kipf2017semisupervised}}   & $85.6 \pm 5.8$        & $76.0 \pm 3.2$ \\
GraphSage {\scriptsize\citep{sage}} & $85.1 \pm 7.6$     & $75.9 \pm 3.2$ \\
SortMPNN  {\scriptsize\citep{davidson2024h}}\hspace{-20pt}     & $\mathbf{90.99 \pm 6.2}$ & \underline{$76.46 \pm 3.68$} \\
AdaptMPNN                     & $90.41 \pm 6.1$      & $75.12 \pm 3.64$  \\
FSW-GNN             &\underline{$90.55 \pm 6.1$} & $\mathbf{76.93 \pm 7.64}$ \\ 
\bottomrule   
SOTA     &\underline{$96.66 \pm 1.23$} & $\mathbf{84.91 \pm 1.62}$ \\ \bottomrule        
\end{tabular}                                  \end{table}

==> tables/table_transductive_learning.tex <==
\begin{table*}[b]
    \caption{Learning accuracy Performance comparison across different datasets and models. Metrics is shown in percents.}
    \label{tab:performance_comparison}
    \centering
    \begin{tabular}{lccccccccc}
        \toprule
        Model      & Cora  & Cite. & Pubm. & Cham. & Squi. & Actor & Corn. & Texa. & Wisc. \\
        \midrule
        GCN  & 85.77 & 73.68 & \underline{88.13} & 28.18 & 23.96 & 26.86 & 52.70 & 52.16 & 45.88 \\
        GAT & \textbf{86.37} & \underline{74.32} & 87.62 & 42.93 & 30.03 & \underline{28.45} & \underline{54.32} & \underline{58.38} & \underline{49.41} \\
        FSW-GNN & \underline{86.35}  & \textbf{75.44} & \textbf{88.17} & \underline{51.18} & \underline{  36.38} & \textbf{34.66} & \textbf{72.43}  & \textbf{75.68} & \textbf{81.56} \\
        Sort-MPNN & 83.46 & 72.69 & 85.15 & \textbf{78.11} & \textbf{74.69} & 31.32 & 67.03 & 70.54 & 73.92 \\
        \hline
        SOTA & \textbf{90.16} & \textbf{82.07} & \textbf{91.31} & \textbf{79.71} & \textbf{76.71} & \textbf{51.81} & \textbf{92.72} & \textbf{88.38} & \textbf{94.99} \\
        \bottomrule
    \end{tabular}
\end{table*}






==> tables/table_wasserstein_approximation_accuracy.tex <==
\begin{table}[htb]
\caption{\label{table_wasserstein_approximation_accuracy}$1$-Wasserstein approximation: Relative error}\label{tab:wasserstein_approximation_error}
    %
    \begingroup
    % Setting the \arraystretch above 1 increases the space between cells.
    % Using \begingroup and \endgroup makes sure that the redefinition
    % of \arraystretch is only local to this table.
    { \fontsize{8}{10}\selectfont
    \renewcommand*{\arraystretch}{1.05}
    \begin{NiceTabular}{lccrrrrrr}
        \toprule
        \Block[c]{1-1}{Dataset} & $d$ & set size & \Block[c]{1-1}{Ours} & PSWE & \Block[c]{1-1}{$\mathcal{N}_{\textup{ProductNet}}$} & \Block[c]{1-1}{WPCE} & \Block[c]{1-1}{$\mathcal{N}_{\textup{SDeepSets}}$} & \Block[c]{1-1}{Sinkhorn}
    \\ \cmidrule(l{2pt}r{2pt}){1-9} 
        noisy-sphere-3   & 3    & 100--299 & \textbf{\SI{1.4}{\percent}} & \SI{2.2}{\percent} & \SI{4.6}{\percent}  & \SI{34.1}{\percent} & \SI{36.2}{\percent} & \SI{18.7}{\percent} 
    \\  noisy-sphere-6   & 6    & 100--299 & \textbf{\SI{1.3}{\percent}} & \SI{1.4}{\percent} & \SI{1.5}{\percent}  & \SI{26.9}{\percent} & \SI{29.1}{\percent} & \SI{13.7}{\percent}
    \\  uniform          & 2    & 256      & \SI{2.4}{\percent} & \textbf{\SI{2.1}{\percent}} & \SI{9.7}{\percent}  & \SI{12.0}{\percent} & \SI{12.3}{\percent} & \SI{7.3}{\percent}
    \\  ModelNet-small   & 3    & 20--199  & \textbf{\SI{2.9}{\percent}} & \SI{5.7}{\percent} & \SI{8.4}{\percent}  & \SI{7.7}{\percent}  & \SI{10.5}{\percent} & \SI{10.1}{\percent}
    \\  ModelNet-large   & 3    & 2047     & \SI{2.6}{\percent} & \textbf{\SI{2.4}{\percent}} & \SI{14.0}{\percent} & \SI{15.9}{\percent} & \SI{16.6}{\percent} & \SI{14.8}{\percent}
    \\  RNAseq           & 2000 & 20--199  & \textbf{\SI{1.1}{\percent}} & \SI{1.2}{\percent} & \SI{1.2}{\percent}  & \SI{47.7}{\percent} & \SI{48.2}{\percent} & \SI{4.0}{\percent}
    \\ \bottomrule
    \end{NiceTabular} }
    \endgroup
    %
    %\floatfoot{\parbox{1\textwidth}{ Mean relative error in approximating the $1$-Wasserstein distance between point sets. }}
    %
    Mean relative error in approximating the $1$-Wasserstein distance between point sets.
\end{table}


==> tables/table_wasserstein_approximation_training_time.tex <==
\begin{table}[htb]
\caption{\label{table_wasserstein_approximation_training_time}$1$-Wasserstein approximation: Training time}\label{tab:wasserstein_approximation_training_time}
    %
    \begingroup
    % Setting the \arraystretch above 1 increases the space between cells.
    % Using \begingroup and \endgroup makes sure that the redefinition
    % of \arraystretch is only local to this table.
    { \fontsize{8}{10}\selectfont
    \renewcommand*{\arraystretch}{1.05}
    \begin{NiceTabular}{lrrrrr}
        \toprule
        \Block[c]{1-1}{Dataset} & \Block[c]{1-1}{Ours} & \Block[c]{1-1}{PSWE} & \Block[c]{1-1}{$\mathcal{N}_{\textup{ProductNet}}$} & \Block[c]{1-1}{WPCE} & \Block[c]{1-1}{$\mathcal{N}_{\textup{SDeepSets}}$}
    \\ \cmidrule(l{2pt}r{2pt}){1-6} 
        noisy-sphere-3   & \SI{2.2}{\minute}  & \SI{33}{\minute} & \SI{6}{\minute} & \SI{1}{\hour} \SI{46}{\minute}  &               \SI{9}{\minute}
    \\  noisy-sphere-6   & \SI{4}{\minute}    & \SI{1}{\hour} & \SI{12}{\minute} &\SI{4}{\hour} \SI{6}{\minute}   & \SI{1}{\hour} \SI{38}{\minute}
    \\  uniform          & \SI{3}{\minute}    & \SI{51}{\minute} & \SI{7}{\minute} &\SI{3}{\hour} \SI{36}{\minute}  & \SI{1}{\hour} \SI{27}{\minute}
    \\  ModelNet-small   & \SI{3}{\minute}    & \SI{48}{\minute} & \SI{7}{\minute} &\SI{1}{\hour} \SI{23}{\minute}  &               \SI{12}{\minute}
    \\  ModelNet-large   & \SI{14.2}{\minute} & \SI{1}{\hour} \SI{19}{\minute} & \SI{8}{\minute} &\SI{3}{\hour} \SI{5}{\minute}   &               \SI{40}{\minute}
    \\  RNAseq           & \SI{4}{\minute}    & \SI{50}{\minute} & \SI{15}{\minute} &\SI{14}{\hour} \SI{26}{\minute} & \SI{3}{\hour} \SI{1}{\minute}
    \\ \bottomrule
    \end{NiceTabular} }
    \endgroup
    %
    %\floatfoot{\parbox{1\textwidth}{ Training times for the different architectures. }}
    %
    Training times for the different architectures.
\end{table}


==> tables/two_tables.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}{0.1\textwidth}
        \centering
        \input{tables/table_lrgb_new}
     %   \caption{\centering Empirical distortion evaluation with respect to the Doubly-Stochastic (DS) metric}
      %  \label{fig_empirical_distortion_ds}
    \end{minipage}
    \hfill
    \begin{minipage}{0.1\textwidth}
   \centering
%\input{figures/tiks_empirical_distortion_vs_tmd.tex}
      %  \vspace{-8pt}
        \input{tables/table_mutag_protein_new} 
       % \vspace{8pt}
     %   \caption{MAD Energy vs. Number of MPNN layers for various models on the Ring long-range task}
      %  \label{fig:oversmoothing}
    \end{minipage}        
\end{figure*}



==> text/acknowledgements.tex <==
\paragraph{Acknowledgements} The authors are partially funded by ISF grant 272/23.
%
We thank Idan Tankel for his technical assistance.


==> text/experiment_chemical_property.tex <==
\paragraph{Chemical property datasets}
In our first experiment, we evaluate FSW-GNN and competing MPNNs on two datasets from LRGB \cite{lrgb2022}. The first, peptides-func, is a multi-label graph classification dataset. The second, peptides-struct, consists of the same graphs as peptides-func but with a regression task. Results in table \ref{tab:lrgb_datasets} show our method reaches comparable but slightly lower accuracy for both tasks. In addition, we add the best results attained by any type of graph neural networks:  \citep{best_func_model} for peptides-func and \cite{best_struct_model} for  peptides-struct.

%Both experiments adhere to the 500K parameter constraint as in \cite{lrgb2022}.
Next, in Table \ref{auc_comparison}, we report AUC results on the  MolHIV dataset for both test and validation sets. In this task, our FSW-GNN is third of the six methods we compare. Interestingly, on the validation set all methods attain significantly better results, and our method outperforms the competing methods. This suggests a non-negligible difference between test and validation distributions in this task.  Also here, we compare to the best (non-MPNN) model known to us for  MolHIV, HyperFusion.



\begin{table}[ht]
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Method} & \textbf{Test AUC} & \textbf{Validation AUC} \\
\hline
GIN & 0.7558 $\pm$ 0.0140 & \underline{0.8232 $\pm$ 0.0090} \\
GIN+FLAG & 0.7654 $\pm$ 0.0114 & 0.8225 $\pm$ 0.0155 \\
GCN & 0.7606 $\pm$ 0.0097 & 0.8204 $\pm$ 0.0141 \\
GCN+FLAG & \underline{0.7683 $\pm$ 0.0102} & 0.8176 $\pm$ 0.0087 \\
GCN+GraphNorm & \textbf{0.7883 $\pm$ 0.0100} & 0.7904 $\pm$ 0.0115 \\
FSW-GNN & 0.76666 $\pm$ 0.01591 & \textbf{0.82542 $\pm$ 0.00821} \\
\hline
Best Model & \textbf{0.8475} &	\textbf{0.8275} \\
\hline
\end{tabular}
\caption{Comparison of Methods based on Test and Validation AUC (mean ± std) in \cite{MolHIV}}
\label{auc_comparison}
\end{table}


==> text/impact_statement.tex <==
%\section*{Impact Statement}
%
%This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.

==> text/reproducibility_statement.tex <==
\paragraph{Reproducibility Statement}
%
All experiments in this paper are fully reproducible. The code for training and evaluation is available in the supplementary material. Reproduction instructions can be found in the file \texttt{readme.md} at the root directory of the downloaded zip file. 
%
For further technical details regarding the experimental setup and parameters, please refer to \autoref{app_numerical_experiments}.

%We have verified that our results are consistent across multiple runs, and the variance across different seeds is reported where applicable. The complete evaluation pipeline and post-processing scripts are included to ensure that the metrics reported in the paper can be reproduced without any modifications.

==> text/sandbox.tex <==
\section*{Sandbox}


\begin{lemma}
    Define $g(\G,\H) = d(\G,\H),f(\G,\H)=||\E(\G)-\E(\H)||$, where $g$ is some 1-WL equivalent piece-wise linear metric, and $\E$ to be a separating piece-wise linear embedding, then by the above lemma, the embedding is actually Bi-lifshiz on any compact set.
\end{lemma}
We need to find piece-wise linear embedding and metric to fulfill the lemma's conditions. Regarding the embedding, assume we have such embedding, and in the following sections, we detail the construction of such embedding denoted by $\E$. Regarding the metric, we now show this metric is indeed piece-wise linear
\ta{I'm not sure whether we need to state this formally in a lemma or not, but for sure we don't need to prove it in the main text.}
We now show that our embedding is \textbf{not} upper lifshiz with respect to $d_{S}$ on a non-bounded domain, but it's lower lifshiz even in the non-bounded domain.  Thus showing a limitation of our metric.
\ta{I wouldn't state in a lemma in the main text that our embedding is not upper lipschitz. I would just this briefly in one or two sentences somewhere at the end of the section, and perhaps refer the reader to further discussion in the appendix.}
\begin{lemma}
     Our embedding is \textbf{not} upper lifshiz with respect to $d_{S}$ on the non-bounded domain, but it's lower lifshiz even in the non-bounded domain.
\end{lemma}
\begin{proof}
 In the appendix we show a series of graphs with $4$ vertices $\{(\G_{n},\H_{n})\}$ such that $d_{S}(\G_{n},\H_{n})\leq 1$ but, $lim_{n\rightarrow \infty}||\E(\G_{n},\H_{n})||=\infty$.
\end{proof}
This example shows that even if the features go to infinity, the distance between graphs can be bounded. In the next metric that is homogenous, this phenomenon can't happen.
\ta{This is for me to write: }
A key component in our GNN 




\ta{It would be more efficient to simply state the main bi-Lipschitzness theorem in the next subsection, then add a short proof-idea paragraph that just says in words that both the embedding and metric are piecewise linear, and state \cref{thm_pwl_ratio_bound}. The full proof with actual lemmas about piecewise linearity is better deferred to the appendix.}
\begin{lemma}
    $d_{S}$ is piece-wise linear when $(A,B)$ are fixed.
\end{lemma}
\begin{proof}
    Note that as $(\A,\B)$ come from a finite set, we can consider them as constants.
    Note that the first expression and the second are point-wise linear as we take $l_1$ norm. Thus, we have a finite number of linear regions, each a polytope.
    Next, note that we minimize a linear function in each linear region; thus, the minimum could be chosen to be at the region's defining points, as if the optimum is in the interior, on the boundary, the value is smaller.
    Thus, there exists a finite number of boundary points and we take minimum over them and a minimum of point-wise linear functions is point-wise linear.
\end{proof}


\ta{This is something we need to think carefully how to present. There is an underlying reason for the lack of upper-Lipschitzness, and it is that our metric becomes too coarse as the features grow in magnitude. We also need to say explicitly that the essential implication of this is that our embedding is \emph{better} than our metric. Then we can close this section  by saying that in the appendix we show that our embedding is bi-Lipschitz with respect to the TMD. }


==> text/subapp_proofs_tmd.tex <==
\subsection{Tree Mover's Distance}
\label{subapp_proofs_tmd}
%
We now prove \cref{thm_tmd_upper_bound}.
\thmTMDUpperBound*

For that, we formalize and prove a useful lemma that will allow us to prove the theorem:
\begin{lemma}
    \label{lemma_td}
    Given two graphs $\G, \H$ and two nodes $i\in \V_{\G}, j \in \V_{\H}$ and denote by $T^{L-1}_{1},T^{L-1}_{2}$ its trees after $L$ iterations and assume that $\X^{L}_{i} = \Y^{L}_{j}$. Then $TMD^{L}(T^{L}_{1},T^{L}_{2}) = 0$.
\end{lemma}
\begin{proof}
    We will prove it by induction on $L$.
    \paragraph{Base} $L$ = $0$ 
    we know from the first element that $\X_{i} = \Y_{j}$ is enough for trees without leaves for zero distance.
    \paragraph{Step}
    Assume that $\X^{L}_{i}=\Y^{L}_{j}$, then, we know that $(\X^{L-1}_{i},E^{L-1},E^{L-1} \cdot d^{\G}_{i})$ = $(\Y^{L-1}_{j},E^{L-1},E^{L-1} \cdot d^{\H}_{j})$. From $\X^{L-1}_{i}=\Y^{L-1}_{j}$, we know the initial feature, thus $|\X_{i}-\Y_{j}| = 0$.
    Denote by $\T^{L-1}_{1},\T^{L-1}_{2}$ the multi-set of trees of nodes $i$ and $j$ in $\G,\H$ respectively. Note that $E^{L-1} \neq 0$ as if $E^{L-1}=0$, all node features of all trees in both graphs are zero as $\E$ is injective, and this contradicts the assumption that no feature is zero. Then, we can reconstruct the multi-set itself of the node features at iteration $L-1$. Thus $\exists \pi: \forall k \in \N^{\G}_{i}, X^{L-1}_{k} = Y^{L-1}_{\pi(k)}$ and by induction assumption, $TM^{L-1}(T^{\G,L-1}_{k},T^{\H,L-1}_{\pi(k)}) = 0, \forall k \in \N_{i}$. Thus the optimal transport $OT(\T^{L}_{},\T^{L}_{2}) = 0$. As we proved also that the features are the same, we have $TMD(\T^{L}_{1},\T^{L}_{2}) = 0$ as desired.
\end{proof}
We now prove the theorem.
\begin{proof}
    Assume that $E^{L}(\G) = E^{L}(\H)$, and we will prove that the metric vanishes after $L$ iterations. 
    We know that there exists a permutation $\pi$ such that $X^{L}_{i} = Y^{L}_{\pi(i)},\forall i \in [n]$.
    By the lemma \ref{lemma_td}, $TD(T^{\G,L}_{i},T^{\H,L}_{\pi(i)}) = 0,\forall i \in [n]$. Thus $TMD^{L}(\G,\H) = 0$ as desired.
\end{proof}


We now show a stability argument that says that if the embedding of two graphs is the same at step $n$ then it's the same for all steps.
\begin{theorem}
    For each two graphs $\G,\H$ there exists $s$ such that if $E^{s}(\G)=E^{s}(\H)$ then $E^{t}(\G)=E^{t}(\H),\forall t\in \NN$. Moreover, the minimal satisfies $s\leq n$.
\end{theorem}
\begin{proof}
    Given iteration $t$, define a stable partition of the nodes such that $u,v$ are equivalent $\iff$. Those nodes have the same initial feature and the same number of neighbors in other partitions. We claim that if the number of colors at iteration $t$ is the same as in iteration $t+1$, then this partition is stable. If not, we have two nodes, such that at iteration $t+1$ will have different colors, and as we concatenate the previous color, the number of colors increases by at least $1$. Thus, we found a stable partition. Thus if $E^{t+1}(\G) = E^{t+1}(\H)$ then $E^{T}(\G) = E^{T}(\H),\forall T>t+1$. Note that a minimal $t$ can be chosen by the pinhole principle to hold $t\leq n$.
\end{proof}

We now prove \cref{thm_tmd_lower_bound}.
\thmTMDLowerBound*

\begin{lemma}
     \label{lemma}
     We will prove first that denote by $T^{L}_{1},T^{ L}_{2}$ the trees defined by $\G,\H$ of nodes $i,j$ respectively after $ L$ iterations then if
    $TD(T^{L}_{1},T^{L}_{2})=0$ then $X^{L}_{i} = Y^{L}_{j}$.
\end{lemma}
\begin{proof}
    By induction on $L$.
    For $L=0$: $TD(T^{0}_{1}, T^{0}_{2})=0$ implies by definition of tree distance that those nodes have the same initial feature.
    \paragraph{Step:} Assume that $TD(T^{ L}_{1},T^{L}_{2})=0$, then denote by $\T_{1}$ the sub-tree collection of $\G$ and by $\T_{2}$ the second one of $\H$.
    We claim both nodes must have the same degree, as otherwise, missing nodes are added by zero padding. All the added sub-trees will have zero features, and the tree distance will be positive, as $0$ is not a valid feature.
    Now, as both nodes have the same degree, by tree distance definition, there exists permutation $\pi$ such that $\forall k\in \N_{i}, TD(T^{\G, L-1}_{k}, T^{\H, L-1}_{\pi(k)}) = 0$ and thus by induction hypothesis: $\X^{L-1}_{k} = \Y^{L-1}_{\pi(k)}$, in addition, $\X^{L-1}_{i} = \Y^{L-1}_{j}$ by hypothesis induction and tree distance zero at level $L$ implies zero distance at level $L-1$. 
    So nodes $i,j$ have the same hidden feature and neighborhood at level $L-1$ so by definition $X^{L}_{i} = Y^{L}_{j}$.
\end{proof}
 We now prove \autoref{second_dir}. 
\begin{proof}
    If $TMD^{L}(\G,\H) = 0$, each node in $\G$ has a corresponding node in $\H$ with tree distance zero, denote this pairing by $\pi$. Thus by the lemma \ref{lemma}, $X^{L}_{i} = Y^{L}_{\pi(i)},\forall i\in \V_{G}$. Thus, at the aggregation at the last level, $E^{L}(\G) = E^{L}(\H)$.
\end{proof}



==> text_backup_Sep_29/abstract.tex <==
\begin{abstract} 
%
% In OpenReview's markdown, the LaTeX command for em-dash --- should be replaced by its explicit unicode character (Alt-0151), or by the math symbol $\unicode{x2014}$.
%


Message-passing neural Networks (MPNNs) for graphs have been used for applications like molecular systems, social networks, and recommendation systems. While the separation power of MPNNs is equivalent to the Weisfeiler-Lehman (WL) test, the quality of separation remains underexplored. 

This paper addresses the issue by seeking bi-Lipschitz continuity guarantees for MPNNs. We demonstrate that, in contrast with summation-based MPNNs which lack bi-Lipschitz properties,  our proposed model provides a bi-Lipschitz embedding on any compact domain with respect to two standard 1-WL-equivalent metrics. Empirically, we show that for long-range tasks our bi-Lipschitz MPNN is significantly more accurate than standard MPNN.

%\nd{suggested alternative: Empirically, we show that for long-range tasks our bi-Lipschitz MPNN is significantly more accurate than standard MPNN. Instead of:} Our theoretical findings are validated on long-range tasks like LRGB and over-squashing tasks without global nodes, showing superior performance.
%
\end{abstract}


==> text_backup_Sep_29/acknowledgements.tex <==
\myparagraph{Acknowledgements} Somebody is funded by somebody. We thank someone for fruitful discussions.

==> text_backup_Sep_29/app_experiment_details.tex <==
\section{Experiment Details}
\label{app_experiment_details}
%
dslsdkldslk

==> text_backup_Sep_29/app_proofs.tex <==
\section{Proofs}
\label{app_proofs}
%
In this section, we prove that none of the proofs were fully proved in the main text.
\subsection{Metric property proof}
\label{metric_property}
We first prove our metric is symmetric and holds the triangle inequality.
The metric is symmetric as if a pair's minimum is obtained at $S$ then the exact value is obtained for the opposite pair with $S^{T}$ and vice-versa. 
We point out that the matrix norm we consider is a sub-multiplicative norm, like the operator norm, Forbinius norm or the $l1$ norm.
Be $(\A,\X),(\B,\Y),(\C,\Z)$ three arbitrary graphs. Then the following holds:
\begin{align*}
   \alpha:= d_{\A,\B} = min_{S\in \Pi_{n}}||\A S-S\B|| +\sum_{i,j}S_{i,j}||\X_{i}-\Y_{j}|| \\
  \beta:= d_{\B,\C} = min_{S\in \Pi_{n}}||\B S-S\C|| +\sum_{i,j}S_{i,j}||\Y_{i}-\Z_{j}||\\
  \gamma:=d_{\A,\C} = min_{S\in \Pi_{n}}||\A S-S\C|| +\sum_{i,j}S_{i,j}||\X_{i}-\Z_{j}||\\
\end{align*}
We want to prove $\gamma \leq \beta+\alpha$. 
The minimum of the first two equations is obtained in $S^{1}, S^{2}$. 
Define $S^{3} = S^{1}\cdot S^{2}$ and note it's also double stochastic.
Then 
\begin{align*}
    ||\A S^{3}-S^{3}\C||=||\A S^{1}S^{2}-S^{1}S^{2}\C||=||\A S^{1}S^{2}-S^{1}\B S^{2}+S^{1}\B S^{2}-S^{1}S^{2}\C|| \\
    \leq 
    ||\A S^{1}S^{2}-S^{1}\B S^{2}|| + ||S^{1}\B S^{2}-S^{1}S^{2}\C|| = 
    ||(\A S^{1}-S^{1}B)\cdot S^{2}|| +
    ||S^{1}\cdot(\B S^{2}-S^{2}\C)||
    \\
    \leq 
    ||S^{2}||\cdot ||\A S^{1}-S^{1}\B|| +
    ||S^{1}||\cdot||\B S^{2}-S^{2}\C|| \leq  ||\A S^{1}-S^{1}\B||+||\B S^{2}-S^{2}\C||
\end{align*}
Next, we show the second part is also smaller:
\begin{align*}
    \sum_{i,j \in [n]}S^{3}_{i,j}\cdot|X_{i}-Y_{j}| =& \sum_{i,j \in [n]}\sum^{n}_{k=1} S^{1}_{i,k}\cdot S^{2}_{k,j} \cdot ||X_{i}-Z_{j}|| \leq \sum_{i,j \in [n]}\sum^{n}_{k=1} S^{1}_{i,k}\cdot S^{2}_{k,j} \cdot (||X_{i}-Z_{k}||+||Z_{k}-Y_{j}||)\\
    =& 
    \sum_{i,j \in [n]}\sum^{n}_{k=1} S^{1}_{i,k} \cdot S^{2}_{k,j} \cdot ||X_{i}-Z_{k}||+\sum_{i,j \in [n]}\sum^{n}_{k=1} S^{1}_{i,k} \cdot S^{2}_{k,j} \cdot ||Y_{j}-Z_{k}|| 
\end{align*}
We now open both sums:
\begin{align*}
    \sum_{i,j \in [n]}\sum^{n}_{k=1} S^{1}_{i,k} \cdot S^{2}_{k,j} \cdot ||\X_{i}-\Z_{k}|| = \sum^{n}_{k = 1}\sum^{n}_{j = 1}\sum^{n}_{i = 1} S^{1}_{i,k} \cdot S^{2}_{k,j} \cdot ||\X_{i} - \Z_{k}||=  \sum_{k}\sum_{j}S^{2}_{k,j}\sum_{i} S^{1}_{i,k} \cdot ||\X_{i} - \Z_{k}|| = \\
    \sum_{k}\sum_{j}S^{2}_{k,j}\cdot f_{k} = \sum_{k}f_{k}\sum_{j}S^{2}_{k,j} = \sum_{k}f_{k} = \sum_{i,j} S^{1}_{i,j}\cdot ||\X_{i} - \Y_{j}||
\end{align*}
With the same argument, we obtain that 
\begin{align*}
    \sum_{i,j}\sum_{k}S^{1}_{i,k}\cdot S^{2}_{k,j}\cdot ||\Y_{j} - \Z_{k}|| = \sum_{i,j} S^{2}_{i,j}\cdot ||\Y_{i} - \Z_{j}||
\end{align*}
So overall we found matrix $S^{3}$ such that:
\begin{align*}
    ||\A S^{3}-S^{3}\C|| +\sum_{i,j}S^{3}_{i,j}||\X_{i}-\Z_{j}|| \leq ||\A S^{1}-S^{1}\B|| +\sum_{i,j}S^{1}_{i,j}||\X_{i}-\Y_{j}||+||\B S^{2}-S^{2}\C|| \\+\sum_{i,j}S^{3}_{i,j}||\Y_{i}-\Z_{j}|| = \alpha + \beta
\end{align*}
We took a specific double stochastic matrix, and the minimum is even smaller, so $\gamma \leq \alpha + \beta$. 
Note that we used the property that $||S\cdot T||\leq ||S||\cdot||T||$ and for each double stochastic matrix $||S||\leq 1$. This holds, for example, in the operator norm or the Forbenius norm.

Now, we show our metric is equivalent to 1-WL.
We begin first with some needed techniques.
\paragraph{Partitions}
Most of our techniques are inspired by \cite{book}.
Given $\G = (\A, \X)$, we define a stable partition $\V = \P_{1}\cup \P_{2}...\cup \P_{k}$ if 
\begin{align}
    \forall u,v \in \P_{i}, \X_{u} =& \X_{v} \\
    \forall l \in [k], |\N_{u}\cap \P_{l}| =& |\N_{v} \cap \P_{l}| 
\end{align}
In simple words, two nodes in the same partition must have the same feature and the same number of neighbors with the same feature.
Note that each singleton is a valid stable partition.
We can characterize a partition as a $k$ tuple, and in the $i'th$ place, we put a tuple of the common feature and a vector telling the number of neighbors in other partitions.
We say that graphs have the same stable partition; if, up to permitting of the $k$ tuple indices, we have the same $k$ tuple. 
\begin{lemma}
    \label{stable}
    The number of colors in 1-WL can't increase at level $n$. In addition, all nodes with the same color at step $n$ make a stable partition.
\end{lemma}
\begin{proof}
     By the pinhole principle, as the number of colors can't decrease, after at most $n$ iterations, the number of different colors will stay the same.  Denote by $\P = (\P_{1},..,\P_{s})$ a partition of the nodes with the same coloring at the $n$ iteration, and be $c\in C$ some color, we claim that nodes in the same partition, have the same number of neighbors with color $c$. As otherwise those nodes that now have same coloring will have different coloring in the next $n+1$ iteration. But as the number of colors doesn't decrease (because of the concatenation of the current color), we have at least one more color, a contradiction. So, we found a stable partition.
\end{proof}
\begin{lemma}
    \label{equivalence}
    The following conditions are equivalent:
    \begin{itemize}
        \item $\G \cong_{1-WL} \H$
        \item Both graphs have a common stable partition.
    \end{itemize}
\end{lemma}
\begin{proof}
    Assume we have the same common partition.
    Up to renaming the names of the vertices of the nodes in the first graphs, we assume we have the same stable partition with the same parameters.
    Assume that a common stable partition exists $\P = \P_{1}\cup..\cup P_{k}$.  
    Then, by simple induction on the number of iterations, we will prove that all nodes in the same partition have the same color in both graphs.
    \newline
    \textbf{Basis} 
    Nodes in the same partition have the same initial feature and, thus, have the same color (in both graphs).
    \newline
    \textbf{Step}
    By the induction hypothesis, all nodes in the same partition iteration $T$ have the same color; 
    and they both have the same number of neighbors with the same color, so the aggregation yields the same output.
    Thus, in iteration $T+1$, those nodes also have the same color.
    Note that this argument is symmetric to both graphs; thus, the 1-WL test will not distinguish them.
    
    On the other hand, if we have the same 1-WL embedding, then we partition the nodes to those classes with the same color at iteration $n$. 
    We have to show this partition is valid.
    First, by definition, those nodes $u,v \in \P_{i}$ have the same node feature (by iteration 1); next, if $u,v$ don't have the same combinatorial degree in $\P_{l}$, then their color won't be the same at iteration $n+1$. But, as shown in lemma \ref{stable}, the number of distinct colors can't increase at iteration $n$. Thus, we found a common stable partition.
\end{proof}
Before proving the following lemma, we revise a definition from \cite{book}.
Given $S \in \R^{n \times n}$, we say $S$ is composable if there exists $P,Q,S_1,S_2$ such that 
\begin{align*}
    S = P \cdot (S_{1} \oplus S_{2}) \cdot Q
\end{align*}
Such that $P,Q$ are permutation matrices.
By simple induction, we can write $M$ as a direct sum of an indecomposable
\begin{align*}
     S = P \cdot (S_{1} \oplus S_{2}\oplus ... \oplus S_{t}) \cdot Q
\end{align*}
\begin{lemma}
    \label{features}
    Be a double stochastic matrix and assume it's in the form of $S = S_{1} \oplus ... \oplus S_{k}$ such that all blocks are indecomposable and $\sum_{i,j}S_{i,j}\cdot||\X_{i}-\Y_{j}||=0$. Denote by $i_{1},...,i_{k+1}$ the indices define the start and the end of $S_{1},...,S_{t}$ and by $I_{k}:=[i_{k},i_{k+1}]$.
    Then $\X_{i}=\Y_{j},\forall t \in [k], \forall i,j \in I_{t}$.
\end{lemma}
\begin{proof}
    Given $t\in [k]$, we build a bipartite graph from $I_{t}$ to itself, such that two indexes $i,j$ are connected if $S_{i,j}>0$. Note that this graph is connected, as otherwise, $S_{t}$ could be composed into its connected components, and thus $S_{t}$ would be composable. 
    Given a path $P = (i_{1},..., i_{l})$ in the graph, note that by definition, as the metric vanishes, and $S_{i_{j}, i_{j+1}}>0$, so $\X_{i_{j}}=\Y_{i_{j+1}}$, thus $\X_{i}=\Y_{j},i\in I_{k},j \in I_{k}$ and we are done.
\end{proof}
\begin{theorem}
    Be $\G,\H$ two featured graphs, then 
    \begin{align*}
        d(\G,\H) = 0 \iff \G =_{1-WL} \H
    \end{align*}
\end{theorem}
We first prove that if the two graphs are 1-WL equivalent, then this metric vanishes. We may assume they have the same stable partition as we proved above. Take $\P=\P_{1}\cup..\cup \P_{t}$, rename the nodes such that they come in consecutive order and denote by $n_{1},n_{2},..,n_{k}$ the sizes of the partitions. Note that by definition, $\forall u,v\in \P_{i}$, both have the same feature and number of neighbors in all $\P_{l}$.
As in the book \cite{book}, define $S:=\frac{1}{n_{1}}J_{n_{1}}\oplus...\oplus\frac{1}{n_{j}}J_{n_{k}}$ and from the book \cite{book}, we know that $\A S=S\B$. As all nodes in the same partition have the same feature, $\X_{i}=\Y_{j},\forall i,j \in I_{k} = [n_{t},n_{t+1}],\forall t \in [k]$, so as $S$ is non-zero only on indexes in the same partition then also this metric vanishes, so also the sum vanishes on $S$. 

For the next direction, be $\G = (\A,\X),\H = (\B,\Y)$ two graphs and assume there exists a matrix of the form of $S=P(S^{1}\oplus...\oplus S_{t})Q$ such that the metric vanishes and denote by $D =S^{1}\oplus...\oplus S_{t}$
We show we can choose $S$ such that it's a block matrix.
\begin{align*}
    ||PDQ\cdot \A - \B \cdot  PDQ|| =& ||P\cdot (DQ\A\cdot Q^{-1}-P^{-1}\B P\cdot D )\cdot Q|| =_{*} ||DQ\A\cdot Q^{-1}-P^{-1}\B P\cdot D||  \\
    \sum_{i,j} S_{i,j} \cdot |\X_{i} - \Y_{j}| =& \sum_{i,j} (PDQ)_{i,j} \cdot |\X_{i} - \Y_{j}| = 
    \sum_{i,j} D_{\pi_{1}^{-1}(i),\pi_{2}(j)} \cdot |\X_{i} - \Y_{j}| = \\
    \sum_{i,j} D_{i,j} \cdot |\X_{\pi_{1}(i)} - \Y_{\pi_{2}^{-1}(j)}|
\end{align*}
(*) - note that the first equality is because permutation matrices preserve the norm.
We define two graphs $\hat{\G} = (Q\A Q^{-1},Q\X)\cong \G, \hat{\H} = (P^{-1}\A P,P^{-1}\Y)\cong \H$.
So, we can choose $S$ to be a diagonal block matrix.
Note that $D$ defines a partition of the nodes, and we will prove that it's a stable partition of both graphs.
From $SA=BS$, we obtain, as in the book \cite{book}, that each of the two nodes $u,v\in \P_{k}$ has the same number of neighbors in $\P_{l},\forall l\in [t]$. 
Next, by the lemma \ref{features}, we know that $\X_{i} = \Y_{j},\forall i,j \in I_{k}$, so nodes in the same partition have the same feature. Thus, this partition is stable.
So, $\hat{\G},\hat{\H}$ have exactly the same partition.
Then $\G,\H$ have the same partition up to isomorphism, and by lemma \ref{equivalence}, both graphs are 1-WL equivalent.



\begin{proof}[Proof of \cref{thm_pwl_ratio_bound}]
    It is enough to prove the left-hand side of \cref{eq_pwl_functions_ratio_bound}. The right-hand side can then be proved by reversing the roles of $f$ and $g$.
    
    Let $A = \setst{x \in M}{g\of{x}>0}$.
    Suppose by contradiction that there exists a sequence $\brc{x_i}_{i=1}^\infty \in A$ such that
    %
    \begin{equation}\label{proof_pwl_ratio_eq_a}
    \frac{f\of{x_i}}{g\of{x_i}} \toas{0}{i\to\infty}.
    \end{equation}
    %
    Since $M$ is compact, we can assume without loss of generality that $x_i \toas{x_0}{i\to\infty} \in M$. Since $g\of{x}$ is bounded on $M$, equation~\cref{proof_pwl_ratio_eq_a} implies that $f\of{x_i}\toas{0}{i\to\infty}$. By continuity, $f\of{x_0} = 0$ and thus $g\of{x_0}= 0$.
    
    Let $L_1,\ldots,L_K \subseteq M$ be the mutual refinement of the linear regions of $f$ and $g$. That is, on each $L_k$, both $f$ and $g$ are linear. Moreover, by a finite number of further refinements, we can assume that all the $L_k$'s are compact convex polytopes. Since there are finitely many $L_k$'s, by taking a subsequence of $\brc{x_i}_{i=1}^{\infty}$, we can assume without loss of generality that all of the $x_i$'s belong to $L_1$. 
    
    Since $f\of{x_0} = g\of{x_0}=0$, the restriction of $f$ and $g$ to $L_1$ can be expressed by 
    %
    \begin{equation}\label{proof_pwl_ratio_eq_b}
        f\of{x} = \bra{a, x-x_0},
        \quad
        g\of{x} = \bra{b, x-x_0},
    \end{equation}
    %
    with $a,b\in \RR^d$ being constant vectors.
    
    Let $v_1,\ldots,v_r$ be the vertices of the convex polytope $L_1$, and let $K \subseteq \RR^d$ be the polyhedral cone generated by $\brc{v_1-x_0,\ldots,v_k-x_0}$ \nd{how is this polyhedral cone defined? conic combinations of $v_i-x_0$? Shouldn't it be conic combinations of $v_i$?}. Thus, $x_0+K \supseteq L_1$, and it is easy to show that any $x \in x_0+K$ that is sufficiently close to $x_0$ belongs to $L_1$.
    Thus:
    %
    \begin{equation}
    \begin{split}        
        0 = & \lim_{i\to\infty}\frac{f\of{x_i}}{g\of{x_i}}
        \geq
        \inf_{x \in L_1 \cap A} \frac{f\of{x}}{g\of{x}}
        =
        \inf_{x \in L_1 \cap A} \frac{\bra{a, x-x_0}}{\bra{b, x-x_0}}        
        \\ \eqx{(a)}&
        \inf_{u \in \br{L_1-x_0} \cap \br{A-x_0}} \frac{\bra{a, u}}{\bra{b, u}}        
        \eqx{(b)}
        \inf_{u \in \br{L_1-x_0} \mid \bra{b,u}>0}
        \frac{\bra{a, u}}{\bra{b, u}}
        \\ \geqx{(c)} &
        \inf_{u \in K \mid \bra{b,u}>0}
        \frac{\bra{a, u}}{\bra{b, u}}
        \eqx{(d)}
        \inf_{u \in K \mid \bra{b,u}=1}
        \bra{a, u},
    \end{split}
    \end{equation}
    %
    where (a) is by change of variables $u=x-x_0$; (b) is since the domains $\br{L_1-x_0} \cap \br{A - x_0}$ and $\setst{u \in L_1 - x_0}{\bra{b,u}>0}$ are identical; (c) holds since $K \supseteq L_1 - x_0$; and (d) holds since $K$ is closed to positive scalar multiplication.

    Therefore, there exists $u_0 \in K$ such that $\bra{b,u}=1$ and $\bra{a,u_0} \leq 0$. Let $\delta > 0$ small enough such that $x_0+\delta u_0 \in L_1$, and thus
    %
    \begin{equation*}
        0 \leq f\of{x_0+\delta u_0} = \bra{a, \br{x_0+\delta u_0} - x_0} = \delta \bra{a,u_0} \leq 0,
    \end{equation*}
    %
    and
    %
    \begin{equation*}
        g\of{x_0+\delta u_0} = \bra{b, \br{x_0+\delta u_0} - x_0} = \delta \bra{b,u_0} = \delta \cdot 1 > 0,
    \end{equation*}    
    %
    which is a contradiction.
\end{proof}

==> text_backup_Sep_29/app_tree_movers_distance.tex <==
\section{Relation to Tree Mover's Distance}
%
This metric, named Tree Mover's distance, denoted by $d_{T}$, is easily seen to be equivalent to 1-WL and comes from \cite{TMD}. This metric is based on a tree distance between the WL computation trees, which can be
written recursively as the sum of the distance between tree roots $r$ and the augmented Wasserstein
between the sub-trees rooting at r’s children.
Assume that the node features come from a domain $\K$ that $0 \notin \K$.

We first review  Wasserstein distances. Recall that if $(\X,d) $ is a metric space, $\Omega \subseteq X$ is a subset,  then we can define the Wasserstein distance on the space  of multisets consisting of $n$ elements in $\Omega$ via
\[
{W}_{1}( x_1,\ldots,x_n, y_1,\ldots,y_n) =\min_{\tau \in S_n} \sum_{j=1}^n d(x_j,y_{\tau(j)})
\]
The augmentation map on multi-sets of size $r\leq n$ is defined as 
$$\rho\left( x_1,\ldots,x_r \right)= (x_1,\ldots,x_r,x_{r+1}=0,\ldots.x_n=0) $$

and the augmented distance on multi-sets of size up to $n$ is defined via
$$W_{d}(X,\hat X)=W_{1}(\rho_{(z)}X,\rho_{(z)}\hat X) $$ 

We now return to define the TMD. We consider the space of graphs $\Gdomain$, consisting of graphs with $\leq n$ nodes, with node features coming from a compact domain $\Omega \subseteq \RR^d$. The TMD is defined using the notion of computation trees:
\begin{definition}
    (Computation Trees). Given a graph $\G=(V,E)$ with node features $\lms x_v \rms_{v\in V} $, let $T_v^1$ be the rooted tree with a single node $v$, which is also the root of the tree, and node features $x_v$. For $K \in \NN$  let $T_v^K$ be the depth-$K$ computation tree of node $v$ constructed by connecting the neighbors of the leaf nodes of $T_v^{K-1}$ to the tree. Each node is assigned the same node feature it had in the original graph $\G$. The multiset of depth-$K$ computation trees defined by $\G$ is denoted by $\mathcal{T}_G^K:=\lms T_v^K \rms_{v\in V}$.
    Additionally, for a tree $T$ with root $r$, we denote by $\mathcal{T}_r$ the multiset of subtrees that root at the descendants of $r$. 
\end{definition}

\begin{definition}
    (Blank Tree). A blank tree $\blankT$ is a tree (graph) that contains a single node and no edge, where the node feature is the blank vector $0$. 
\end{definition}
Recall that by assumption, all node features will come from the compact set $\Omega$, and $0 \not \in \Omega$. 



We can now define the tree distance:
\begin{definition}
    (Tree Distance).\footnote{Note the difference from the original definition in \cite{chuang2022tree} is due to our choice to set the depth weight to 1 and using the 1-Wasserstein which is equivalent to optimal transport} 
    The distance between two trees $T_a, T_b$ with features from $\Omega$ and $0\not \in \Omega$, is defined recursively as
    \[
    TD(T_a, T_b) := \begin{cases}
      \|x_{r_a}-x_{r_b}\|_1 + W_{TD}^{\blankT} (\mathcal{T}_{r_a}, \mathcal{T}_{r_b}) & \text{if $K>1$} \\
      \|x_{r_a}-x_{r_b}\|_1 & \text{otherwise}  
    \end{cases}
    \]
    where $K$ denotes the maximal depth of the trees $T_a$ and $T_b$. 
\end{definition}

\begin{definition}
    (Tree Mover's Distance). Given two graphs, $G_a, G_b$ and $w,K \ge 0$, the tree mover's distance is defined as 
    \[
    TMD^K(G_a, G_b) = W^{\blankT}_{TD}(\mathcal{T}_{G_a}^K, \mathcal{T}_{G_b}^K)
    \]
\end{definition}
where $\mathcal{T}_{G_a}^K$ and $\mathcal{T}_{G_b}^K$ denote the multiset of all depth $K$ computational trees arising from the graphs $G_a$ and $G_b$, respectively. 
We refer the reader to \cite{chuang2022tree}, where they prove this is a pseudo-metric that fails to distinguish only graphs that cannot be separated by $K+1$ iterations of the WL test.


Note to the following properties:
\begin{itemize}
    \item The metric is 1-WL equivalent if $0$ is not a valid node feature. 
    \item  $TMD^K((\A, \alpha \cdot \X),(\B, \alpha \cdot \Y)) = \alpha \cdot TMD^K(\X,\Y)$
    \item The metric is point-wise linear in $\X,\Y$.
\end{itemize}
Note that those properties are equivalent to saying that the metric is 1-WL equivalent, homogeneous.
We now present an embedding that $\E$ that is Bilifshiz with respect to the TMD metric in any domain.
We now define our embedding and show the desired properties for lemma \ref{thm_pwl_ratio_bound}.
\begin{align*}
    \X^{0}_{i} =& \X_{i} \\
    E^{t} =& \E(\{\{\X^{t}_{j}|j\in N_{i}\}\}) \\
    \X^{t+1}_{i} &= (\X^{t}_{i},E^{t},E^{t} \cdot d_{i}) \\
    \E^{T}(\G) =& \E(\{\{\X^{T}_{1},..,\X^{T}_{n}\}\})
\end{align*}
We now show that if two graphs have the same embedding at time step $L$, their $TMD^{L}$ vanishes.
\begin{theorem}
    Be $L$ some integer.
    Assume that $E^{L}(\G) = E^{L}(\H)$ then $TMD^{L}(\G,\H) = 0$.
\end{theorem}
For that, we formalize and prove a useful lemma that will allow us to prove the theorem:
\begin{lemma}
    \label{lemma_td}
    Given two graphs $\G, \H$ and two nodes $i\in \V_{\G}, j \in \V_{\H}$ and denote by $T^{L-1}_{1},T^{L-1}_{2}$ its trees after $L$ iterations and assume that $\X^{L}_{i} = \Y^{L}_{j}$. Then $TMD^{L}(T^{L}_{1},T^{L}_{2}) = 0$.
\end{lemma}
\begin{proof}
    We will prove it by induction on $L$.
    \paragraph{Base} $L$ = $0$ 
    we know from the first element that $\X_{i} = \Y_{j}$ is enough for trees without leaves for zero distance.
    \paragraph{Step}
    Assume that $\X^{L}_{i}=\Y^{L}_{j}$, then, we know that $(\X^{L-1}_{i},E^{L-1},E^{L-1} \cdot d^{\G}_{i})$ = $(\Y^{L-1}_{j},E^{L-1},E^{L-1} \cdot d^{\H}_{j})$. From $\X^{L-1}_{i}=\Y^{L-1}_{j}$, we know the initial feature, thus $|\X_{i}-\Y_{j}| = 0$.
    Denote by $\T^{L-1}_{1},\T^{L-1}_{2}$ the multi-set of trees of nodes $i$ and $j$ in $\G,\H$ respectively. Note that $E^{L-1} \neq 0$ as if $E^{L-1}=0$, all node features of all trees in both graphs are zero as $\E$ is injective, and this contradicts the assumption that no feature is zero. Then, we can reconstruct the multi-set itself of the node features at iteration $L-1$. Thus $\exists \pi: \forall k \in \N^{\G}_{i}, X^{L-1}_{k} = Y^{L-1}_{\pi(k)}$ and by induction assumption, $TM^{L-1}(T^{\G,L-1}_{k},T^{\H,L-1}_{\pi(k)}) = 0, \forall k \in \N_{i}$. Thus the optimal transport $OT(\T^{L}_{},\T^{L}_{2}) = 0$. As we proved also that the features are the same, we have $TMD(\T^{L}_{1},\T^{L}_{2}) = 0$ as desired.
\end{proof}
We now prove the theorem.
\begin{proof}
    Assume that $E^{L}(\G) = E^{L}(\H)$, and we will prove that the metric vanishes after $L$ iterations. 
    We know that there exists a permutation $\pi$ such that $X^{L}_{i} = Y^{L}_{\pi(i)},\forall i \in [n]$.
    By the lemma \ref{lemma_td}, $TD(T^{\G,L}_{i},T^{\H,L}_{\pi(i)}) = 0,\forall i \in [n]$. Thus $TMD^{L}(\G,\H) = 0$ as desired.
\end{proof}
This proves that our embedding is stronger than the metric.
We now show a stability argument that says that if the embedding of two graphs is the same at step $n$ then it's the same for all steps.
\begin{theorem}
    For each two graphs $\G,\H$ there exists $s$ such that if $E^{s}(\G)=E^{s}(\H)$ then $E^{t}(\G)=E^{t}(\H),\forall t\in \NN$. Moreover, the minimal satisfies $s\leq n$.
\end{theorem}
\begin{proof}
    Given iteration $t$, define a stable partition of the nodes such that $u,v$ are equivalent $\iff$. Those nodes have the same initial feature and the same number of neighbors in other partitions. We claim that if the number of colors at iteration $t$ is the same as in iteration $t+1$, then this partition is stable. If not, we have two nodes, such that at iteration $t+1$ will have different colors, and as we concatenate the previous color, the number of colors increases by at least $1$. Thus, we found a stable partition. Thus if $E^{t+1}(\G) = E^{t+1}(\H)$ then $E^{T}(\G) = E^{T}(\H),\forall T>t+1$. Note that a minimal $t$ can be chosen by the pinhole principle to hold $t\leq n$.
\end{proof}
We now show the opposite: if the metric vanishes at some step, it implies equal embedding at the same step.
\begin{theorem}
    \label{second_dir}
    Assume we are given two graphs with the same number of nodes, and $k\in \NN$ such that $TMD^{k}_{T}(\G,\H) = 0$ then $E^{k}(\G) = E^{k}(\H)$. 
\end{theorem}
\begin{lemma}
     \label{lemma}
     We will prove first that denote by $T^{L}_{1},T^{ L}_{2}$ the trees defined by $\G,\H$ of nodes $i,j$ respectively after $ L$ iterations then if
    $TD(T^{L}_{1},T^{L}_{2})=0$ then $X^{L}_{i} = Y^{L}_{j}$.
\end{lemma}
\begin{proof}
    By induction on $L$.
    For $L=0$: $TD(T^{0}_{1}, T^{0}_{2})=0$ implies by definition of tree distance that those nodes have the same initial feature.
    \paragraph{Step:} Assume that $TD(T^{ L}_{1},T^{L}_{2})=0$, then denote by $\T_{1}$ the sub-tree collection of $\G$ and by $\T_{2}$ the second one of $\H$.
    We claim both nodes must have the same degree, as otherwise, missing nodes are added by zero padding. All the added sub-trees will have zero features, and the tree distance will be positive, as $0$ is not a valid feature.
    Now, as both nodes have the same degree, by tree distance definition, there exists permutation $\pi$ such that $\forall k\in \N_{i}, TD(T^{\G, L-1}_{k}, T^{\H, L-1}_{\pi(k)}) = 0$ and thus by induction hypothesis: $\X^{L-1}_{k} = \Y^{L-1}_{\pi(k)}$, in addition, $\X^{L-1}_{i} = \Y^{L-1}_{j}$ by hypothesis induction and tree distance zero at level $L$ implies zero distance at level $L-1$. 
    So nodes $i,j$ have the same hidden feature and neighborhood at level $L-1$ so by definition $X^{L}_{i} = Y^{L}_{j}$.
\end{proof}
 We now prove \autoref{second_dir}. 
\begin{proof}
    If $TMD^{L}(\G,\H) = 0$, each node in $\G$ has a corresponding node in $\H$ with tree distance zero, denote this pairing by $\pi$. Thus by the lemma \ref{lemma}, $X^{L}_{i} = Y^{L}_{\pi(i)},\forall i\in \V_{G}$. Thus, at the aggregation at the last level, $E^{L}(\G) = E^{L}(\H)$.
\end{proof}
We now show a stability property of the TMD metric.
\begin{theorem}
    For each two graphs $\G,\H$ there exists $s$ such that if $d^{t}_{T}(\G,\H)=0,\forall t\in[s]$ then $d^{t}_{T}(\G,\H)=0,\forall t\in \NN$. Moreover, the minimal $s\leq n$
\end{theorem}
\begin{proof}
    From \autoref{second_dir}, we know that if $d^{n}_{T}(\G,\H) = 0$ then $E^{n}(\G)=E^{n}(\H)$ and thus $E^{T}(\G)=E^{T}(\H),\forall T\in \NN$, thus $d^{T}_{T}(\G,\H) = 0,\forall T\in \NN$.
\end{proof}
If we take the embedding to be the embedding at step $n$ and the metric to be the TMD at depth $n$ and $\K$ to be a convex feature domain not containing $0$, then the embedding is Bi-lifshiz with respect to it.
\ys{Not clear.}
\begin{theorem}
    Our embedding $\E^{n}$ is Bilifshiz with respect to the $TMD_{n}$ metric on any domain.
\end{theorem}
\begin{proof}
    First, note that the functions are piece-wise linear. Next, if $\E^{n}(\G) = \E^{n}(\H)$ then, $d^{n}(\G,\H)=0$. on the other hand, if $d^{n}(\G,\H)=0$ then $\E^{n}(\G) = \E^{n}(\H)$. Now, we show we can use a compact domain to show bi-lifshizness
     \begin{equation}
    Sup_{|\Y|\leq|\X|}\frac{|E^{n}(A,X)-E^{n}(B,Y)|}{d^{n}_{T}((A,X),(B,Y))} = 
    Sup_{|Y|\leq|X|=1}\frac{|E^{n}(A,X/|X|)-E^{n}(B,Y/|X|)|}{d^{ n}_{T}((A,X/|X|),(B,Y/|X|))}
    \end{equation}
    And the same is for infimum. As the second domain is compact and convex, the supremum is bounded above and the infimum below. 
\end{proof}


==> text_backup_Sep_29/general_comments.tex <==
\newpage
\section*{General Comments}
\begingroup
\color{blue}
%
\begin{itemize}
\item When you cite other papers, remember to use \texttt{\textbackslash citep} and \texttt{\textbackslash citep} correctly. 
%
\item For multisets, use the macro \texttt{\textbackslash multiset}, not ${{}}$. It looks better: $\multiset{\bx[1],\ldots,\bx[n]}$
%
\item It's Lipschitz
%
\end{itemize}

This section disappears when you disable \texttt{show\_our\_comments}.

\endgroup



==> text_backup_Sep_29/sandbox.tex <==
\section*{Sandbox}

==> text_backup_Sep_29/sec_conclusion.tex <==
\section{Conclusion}
\label{sec_conclusion}
%
In conclusion, ...

==> text_backup_Sep_29/sec_introduction.tex <==
\section{introduction}
\label{sec_introduction}
%


Graph neural networks are a central research topic in contemporary machine learning research, with a multitude of different models being proposed. Many of the most popular models, such as GraphSage \cite{XXX}, GAT \cite{XXX}, and GCN \cite{XXX}, can be seen as an instantiation of Message Passing Neural Networks (MPNNs) \cite{Gilmer2017NeuralMP}. 

A well known limitation of MPNNs is that they cannot differentiate between all distinct graphs. In fact, a pair of distinct graphs which cannot be separated by the Weisfeiler-Lehman (WL) graph isomorphism test will not be separated by \emph{any} MPNN  \cite{xu2018how}. Conversely, it is shown in \cite{xu2018how,morris2019WL} that suitably chosen MPNN will be able to separate all pairs of graphs which are separable by WL. We will say that such an MPNN is WL-equivalent. 

Recent work had shown that WL-equivalent MPNN can be unrealistically small \cite{amir2023neural,XXX}. For these MPNN, it was observed that the separation of graphs is so  weak that extra precision digits are needed to observe it \nd{(see XXXanalytic,snir)}. Furthermore, MPNN often suffer from  oversmoothing \nd{cite}, where  distinct nodes are assigned near-identical node features.  These two observations motivate the development of \emph{quantitative} estimate of MPNN separation, by means of 
bi-Lipschitz stability guarantees. These guarantees would ensure that  euclidean distances in the MPNN feature space are neither much larger nor much smaller than distances in the original graph-space, which are defined by a suitable graph-metric (defined up to WL equivalence).

The notion of 
Bi-Lipschitz stability analysis is common in various fields \cite{XXX}, and has been recently become a topic of interest in the GNN community as well. Indeed, a recent survey \cite{XXX} identified bi-Lipschitz guarantees for MPNNs as a key challenge for future GNN research. 

Some first steps towards addressing these challenges have already been made. It has been observed in \cite{XXXjegelka,XXXyair} that many MPNN models are upper-Lipscitz. However, essentially all popular MPNN models, such as those based on sum-pooling, are not lower-Lipschitz continuous \cite{davidson2024h}. In contrast, \cite{davidson2024h} propose a new MPNN, based on sorting-based aggregations from \cite{balan2022permutation}, which \emph{is} bi-Lipschitz \emph{in expectation}, a weaker notion than the standard bi-Lipschitz definition. 

\nd{In this paper... stopped here}  






\nd{I will continue working on intro and related work on Sunday. Also will add the missing citations}
% Motivated by  applications for chemoinformatics \cite{Gilmer2017NeuralMP}, social networks \cite{borisyuk2024lignn},
% and recommendation systems \cite{gao2023survey}, and more, permutation invariant deep learning for 
% graphs has gained increasing interest in recent years. This, in turn, has inspired several theoretical
% works that analyze common GNNs and their expressive power and limitations.
%  Our focus in this paper will be on Message Passing Neural Network (MPNN) \cite{Gilmer2017NeuralMP} paradigm, which includes a variety of popular GNNs \cite{xu2018how, Gilmer2017NeuralMP, kipf2017semisupervised}. In their seminal works, \cite{xu2018how, morris2019WL} prove that MPNNs are at most expressiveness as the Weisfeiler-Lehman (WL) graph isomorphism test \cite{weisfeiler1968reduction}.
% Accordingly, maximally expressive MPNNs are those that can separate all graph pairs that
% are WL-separable. \cite{xu2018how, morris2019WL} shows that MPNNs that employ injective multi-set functions are maximally expressive. Examples of MPNNs that are 1-WL equivalent are \cite{gin}.
% However, while current theory ensures separation, it tells us little about the separation quality, so that embeddings of "separable" objects may
% be highly similar, to the extent that in some cases, graphs that can be theoretically separated by
% maximally expressive MPNNs are completely identical on a computer with fixed finite precision (see
% \cite{bravo2024dimensionality}, figure 1). To study the separation quality of permutation invariant models, we will search for bi-lifshiz continuity guarantees. \cite{amir2023neural} showed summation-based aggregation functions are not bi-lifshiz with respect to the distance between multi-sets;\ta{We actually did it in \citep{amir2023neural}} thus, all summation-based GNNs are not bi-lifshiz. Recently \cite{davidson2024h} presented a network that is a bi-lifhsiz on expectation over weights drawn uniformly from the circle. In this work, we show a Bi-lifshiz embedding on any compact domain(not in expectation) with respect to a metric equivalent to 1-WL.

% We demonstrate our theoretical superiority on long-range tasks like LRGB \cite{lrgb2022}, short-range tasks like Cora \cite{cora}, and over-squashing tasks taken from \cite{alon, bron} without global nodes.

\inputtext{subsec_related_works}

==> text_backup_Sep_29/sec_main_contributions.tex <==
\section{Main Contributions}
\label{sec_main_contributions}
%
In this section, we outline our main contributions. First we describe our proposed metric for vertex-featured graphs. Then we present our bi-Lipschitz GNN, and discuss its theoretical properties.
%

%\subsection{WL-equivalent metric for vertex-featured graphs}
%\label{subsec_metric}
%
We start by describing our proposed metric and then show that it is equivalent to the WL test for vertex-featured graphs.
%
Our metric is inspired by the work of \citet{book}, who defined a metric for featureless graphs with a fixed number of vertices. Let $G$ and $\tilde G$ be two graphs, each with $n$ vertices, and let their corresponding adjacency matrices be $A$ and $\tilde A$. Their metric is defined as
%
\begin{equation}\label{eqdef_metric_ds_nofeat}
    \rho\of{G,\tilde G}
    =
    \min_{S\in\D_n} \ 
    \norm{AS-S\tilde A},
\end{equation}
%
where $\D_n$ is the space of all $n\times n$ doubly-stochastic matrices, and $\norm{\argdot}$ is an arbitrary operator norm. They also proved that this metric assigns zero distance to two graphs if and only if they are WL-indistinguishable.

Building on this idea, we adapt the above metric to vertex-featured graphs with varying numbers of vertices, by augmenting it as follows:
%
\begin{equation}\label{eqdef_metric_ds}
    \rhods\of{G,\tilde G}
    =
    \abs{n-\tilde n}
    +
    \min_{S\in\Pi\of{n,\tilde n}} \ 
    \norm{AS-S\tilde A}
    +
    \sum_{i\in\brs{n}, j\in\brs{\tilde n}} s_{ij}
    \norm{\bx_i-\btx_j},
\end{equation}
%
where: 
(1) $n=\abs{V}$, $\tilde n = \abs{\tilde V}$; (2) $\Pi\of{n,\tilde n}$ is the set of $n \times \tilde n$ matrices $S$ that satisfy $\sum_{j=1}^{\tilde n} S_{ij} = \tfrac{1}{n}$, $\sum_{i=1}^{n} S_{ij} = \tfrac{1}{\tilde n}$;
(3) $\bx_i$ and $\btx_j$ denote the vertex features of $G$ and $\tilde G$ respectively. The norms in \cref{eqdef_metric_ds} can be arbitrary. In the rest of this paper we use $\norm{\argdot}$ to denote the $\ell_2$ norm for vectors and entrywise $\ell_2$ norm for matrices.

%The following theorem states that $\rhods\of{\argdot,\argdot}$ is indeed a WL-equivalent metric. A proof is in the appendix.\ta{add reference}
%
\begin{theorem}[Proof in \cref{metric_property}]
    Let $\rhods: \GNd \times \GNd \to \RR_{\geq 0}$ be as in \cref{eqdef_metric_ds}.
    Then $\rhods$ is a WL-equivalent metric.
    %Let $G,\tilde G \in \GNd$. Then $\rhods\of{G,\tilde G} = 0$ if and only if $G \wleq \tilde G$.
\end{theorem}

\ta{Here maybe say something good about our metric. e.g.:}
The metric $\rhods$ provides a natural measure to quantify the difference between two graphs with vertex features. When taking the norms to be $\ell_1$ norms, it can be computed easily by a linear programming solver.

%\ta{State something like this when we're chosen the norm and we're sure of the complexity: }
%
%The metric $\rhods$ is defined by a linear program that can be solved in $\O\of{\argdot}$ time, which matches the complexity of the WL test. However, unlike WL, here the outcome not only determines whether two vertex-featured graphs are WL-equivalent or not, but also quantifies the extent to which they are inequivalent.


%\subsection{Bi-Lipschitz Embedding and Graph Neural Network}
%\label{subsec_bilipschitz_gnn}
%
We now present our main contribution: a novel MPNN with WL-equivalent separation power for vertex-featured graphs. Unlike other MPNNs in this class, this MPNN maps input graphs into the output Euclidean space in a bi-Lipschitz manner, both with respect to the metric $\rhods$ and the Tree Mover’s Distance. 

The core innovation in our MPNN lies in its message aggregation method. As discussed in \cref{sec_problem_setting}, most prevalent MPNNs aggregate messages using simple pooling operations such as sum- or max-pooling. However, theoretical analyses in recent years have revealed significant limitations in these methods. \citet{amir2023neural} showed that sum-pooling inevitably induces infinite distortion on its input space, thereby making bi-Lipschitzness impossible; see also \citep{cahill2023bilipschitz} for a related result.\ta{Is this the proper way to cite Cahill?} Furthermore, \citet{xu2018how} showed that max-pooling is not even injective, as it fails to account for repetitions of multiset elements. These findings suggest that traditional pooling methods may pose a substantial bottleneck in the performance of MPNNs.

More sophisticated pooling methods have been proposed in recent works.
%
\citet{davidson2024h} proposed an MPNN and proved that it is 2-Holder in expectation. Although they did not prove this in their paper, it can be shown that their MPNN is bi-Lipschitz. However, their pooling mechanism requires a priori knowledge of the highest possible vertex degree in the input graphs, which is a significant limitation. Other pooling mechanisms were proposed in \citet{fspool,naderializadeh2021pooling}, but their methods do not have bi-Lipschitzness guarantees. \ta{Cite Balan? He did not discuss MPNNs in his work. e.g. Similarly, a pooling method based on sorting was proposed by Balan et al., but it only accommodates multisets of fixed size, and thus is only applicable to regular graphs.}

%\ta{Cite Yair's work and other works that used bi-Lipschitz embeddings (Kolouri? FSpool? Balan?)} \nd{indeed. Especially Yair. Need to explain similarities and differences. I would emphasize the issue of varying cardinalities. Also mention  'in expectation' but say yair also is probably bi-lipschitz in the standard sense, he just didn't prove it.}


To address these limitations, we build on the recent work of \citet{amir2024injective}, who proposed the \emph{Fourier Sliced-Wasserstein (FSW) embedding} for multisets. In a nutshell, this embedding operates by taking random one-dimensional projections (called \emph{slices}) of the input multiset, calculating the quantile function for each slice, and sampling its Fourier transform at a random frequency. Importantly, they proved that this embedding is bi-Lipschitz with respect to the Wasserstein distance. This property ensures better numerical retention of information, making the FSW embedding a potentially superior candidate for multiset aggregation. Our proposed architecture, which we name \textbf{FSW-GNN}, leverages the FSW embedding as its message aggregation mechanism. We now provide a formal description. 

The FSW embedding $\embfsw\of{\argdot}$ takes input multisets over $\RR^d$ and maps them into a Euclidean space $\RR^m$. It depends on parameters that are drawn randomly from a specific distribution; see \citep{amir2024injective} for more details. It was shown that with a sufficiently large $m$, with probability 1 the resulting embedding is bi-Lipschitz with respect to the Wasserstein distance.

The FSW-GNN processes input graphs $G=\br{V,E,X}$ by $T$ message-passing iterations according to the following recursive formula:
%
\begin{equation}\label{eqdef_fswgnn}
\begin{split}
    \bh^{\br{0}}_{v} \eqdefx & \bx_{v},
    %\quad v \in V, 
    %
    \\ \bq_v^{\br{t}} 
    \eqdefx &
    \embfswt[t]\of{ \setst{ \bh^{\br{t-1}}_u } {u \in \N_v} }, 
    \quad 1 \leq t \leq T
    \\ \bh^{\br{t}}_v
    \eqdefx &
    \Phi^{\br{t}} \of{ \brs{\bh^{\br{t-1}}_v;\bq^{\br{t}}_v}},
\end{split}
\end{equation}
%
where the functions $\embfswt[t]$ are all instances of the FSW embedding,
% with output dimension $m$, to be determined later;
% $\bM^{\br{t}}$ are matrices with random \nd{learned}\ta{not in the embedding} coefficients, all of whose output dimension is $m$;
% 
$\Phi^{\br{t}}$ are MLPs,
and $\brs{\bx; \by}$ denotes column-wise concatenation of column vectors $\bx$ and $\by$. Finally, a graph-level output is computed by:
%
\begin{equation}\label{eqdef_fswgnn_readout}
    \bh_G \eqdef 
    \Psi \circ
    \embfswglob\of{\setst{ \bh^{\br{T}}_v}{v\in V}},
\end{equation}
%
where, again, $\embfswglob$ is an FSW embedding, and $\Psi$ is an MLP.

The following \lcnamecref{thm_fswgnn_is_wl_equivalent} shows that with the appropriate choice of MLP sizes and number of iterations $T$, our proposed architecture has the separation power of the WL test.
%
\begin{theorem}\label{thm_fswgnn_is_wl_equivalent}
    %Consider the space of vertex-featured graphs $\GNof\Omega$ over the feature domain $\Omega\subset\RR^d$, and suppose that $\Omega$ is compact.
    Consider the FSW-GNN architecture defined in \cref{eqdef_fswgnn,eqdef_fswgnn_readout} for input graphs in $\GNd$, with $T=N$ iterations, all MLPs being one-layer matrices with output dimension $m \geq 2Nd+2$ and no activation, and all FSW embeddings having output dimension $m$. Suppose all FSW embeddings are initialized independently at random, and all MLPs have random entries drawn from an absolutely-continuous distribution over $\RR$. 
    Then with probability 1, the following holds: For any pair of graphs $G, \tilde G \in \GNd$, the corresponding outputs $\bh_G$ and $\bh_{\tilde G}$ computed by the FSW-GNN are equal if and only if $G \wleq \tilde G$.
\end{theorem}
%
%The probability in \cref{thm_fswgnn_is_wl_equivalent} is over the matrices $\bM^{\br{t}}$ and embedding functions $\embfswt[t]$ and $\embfswglob$, which depend on random parameters. 
%Note that the theorem does not require all embedding functions to be generated independently. In fact, two instances suffice: one for $\embfswt[1]$, which maps input multisets in $\RR^d$ into a single vector in $\RR^m$, and another instance for all $\embfswt[t]$ with $2 \leq t \leq T$ and for $\embfswglob$, all of which map input multisets in $\RR^m$ into a single vector in $\RR^m$.

The proof of \cref{thm_fswgnn_is_wl_equivalent} is based on the study of $\sigma$-subanalytic functions and the \emph{Finite Witness Theorem}, introduced in \citep{amir2023neural}.

It is worth noting that the output dimension $m$ required in practice is typically considerably lower than the one required in \cref{thm_fswgnn_is_wl_equivalent}. This can be explained by the following fact: If all input graphs come from a sub-manifold of $\GNd$ with intrinsic dimension $D$ significantly lower than the ambient dimension $n\cdot d$, then it can be shown that $m=2D+2$ suffices for WL-equivalence.


\paragraph{From separation to bi-Lipschitzness}
%
We now show that the WL-equivalence property of the FSW-GNN implies that it is in fact bi-Lipschitz, as stated in the following theorem.

\begin{theorem}\label{thm_fswgnn_is_bilip}
Let $\Omega \subset \RR^d$ be compact. Then under the assumptions of
\cref{thm_fswgnn_is_wl_equivalent}, the FSW-GNN is bi-Lipschitz with respect to $\rhods$ and TMD on $\GNof\Omega$.
\end{theorem}
\ta{A. Note that strictly speaking, the TMD part is true only if we augment all vertex feature vectors with a coordinate of 1. B. I skipped the part of bi-Lipschitzness without compactness assumption. This is too complex for the main text.} \nd{good}

We now give a high-level explanation of the proof idea. The full proof is in the appendix. \ta{verify}
%
To prove \cref{thm_fswgnn_is_bilip}, we rely on the following facts: (1) the output of FSW-GNN for an input graph $G=\br{V,E,X}$ is piecewise-linear with respect to the vertex-feature matrix $X$. This follows from properties of the FSW embedding functions used in \cref{eqdef_fswgnn,eqdef_fswgnn_readout}. (2) both metrics $\rhods$ and TMD can be transformed, with bounded distortion, into  piecewise-linear metrics by choosing all the vector norms they employ to be the $\ell_1$ norm. The claim them follows from these observations and the following \lcnamecref{thm_pwl_ratio_bound}:
%
\begin{lemma}
\label{thm_pwl_ratio_bound}
    Let $f,g: M \to \RR_{\geq 0}$ be non-negative piece-wise-linear functions defined on a compact polygon $M \subset \RR^d$. Suppose that for all $x\in M$, $f(x) = 0$ if and only if $g(x)=0$. Then there exist real constants $c,C > 0$ such that
    \begin{equation}\label{eq_pwl_functions_ratio_bound}
        c \cdot g\of{x} \leq f\of{x} \leq C \cdot g\of{x}
    \end{equation}
    for all $x \in M$ for which $g\of{x}>0$.
\end{lemma}

% The rest of the proof is as follows: Let $G,\tilde G \in \GNof\Omega$, $G=\br{V,E,X}$ and $\tilde G=\br{\tilde V, \tilde E, \tilde X}$, with $n$ and $\tilde n$ vertices respectively. It is enough to show that the bi-Lipschitz ratio is bounded on all choices of $X \in \Omega^n$, $\tilde X \in \Omega^{\tilde n}$, since there is a finite number of choices of $n,\tilde n \leq N$ and edges $E$, $\tilde E$. Define the function $f\of{X,\tilde X} = \norm{\bh_G - \bg_{\tilde G}}_1$, $g\of{X,\tilde X} = \rho\of{G,\tilde G}$, where $\rho$ is either $\rhods$ or TMD. By the comment above, both $f$ and $g$ are piecewise linear. Since both FSW-GNN and the metric $\rho$ are WL-equivlanet, $f$ and $g$ have the same zero set. Thus, \cref{thm_pwl_ratio_bound} guarantees the existence of Lipschitz constants $c,C$. Q.E.D.

\redline{End of Section}

\begin{lemma}
    Define $g(\G,\H) = d(\G,\H),f(\G,\H)=||\E(\G)-\E(\H)||$, where $g$ is some 1-WL equivalent piece-wise linear metric, and $\E$ to be a separating piece-wise linear embedding, then by the above lemma, the embedding is actually Bi-lifshiz on any compact set.
\end{lemma}
We need to find piece-wise linear embedding and metric to fulfill the lemma's conditions. Regarding the embedding, assume we have such embedding, and in the following sections, we detail the construction of such embedding denoted by $\E$. Regarding the metric, we now show this metric is indeed piece-wise linear
\ta{I'm not sure whether we need to state this formally in a lemma or not, but for sure we don't need to prove it in the main text.}
We now show that our embedding is \textbf{not} upper lifshiz with respect to $d_{S}$ on a non-bounded domain, but it's lower lifshiz even in the non-bounded domain.  Thus showing a limitation of our metric.
\ta{I wouldn't state in a lemma in the main text that our embedding is not upper lipschitz. I would just this briefly in one or two sentences somewhere at the end of the section, and perhaps refer the reader to further discussion in the appendix.}
\begin{lemma}
     Our embedding is \textbf{not} upper lifshiz with respect to $d_{S}$ on the non-bounded domain, but it's lower lifshiz even in the non-bounded domain.
\end{lemma}
\begin{proof}
 In the appendix we show a series of graphs with $4$ vertices $\{(\G_{n},\H_{n})\}$ such that $d_{S}(\G_{n},\H_{n})\leq 1$ but, $lim_{n\rightarrow \infty}||\E(\G_{n},\H_{n})||=\infty$.
\end{proof}
This example shows that even if the features go to infinity, the distance between graphs can be bounded. In the next metric that is homogenous, this phenomenon can't happen.
\ta{This is for me to write: }
A key component in our GNN 




\ta{It would be more efficient to simply state the main bi-Lipschitzness theorem in the next subsection, then add a short proof-idea paragraph that just says in words that both the embedding and metric are piecewise linear, and state \cref{thm_pwl_ratio_bound}. The full proof with actual lemmas about piecewise linearity is better deferred to the appendix.}
\begin{lemma}
    $d_{S}$ is piece-wise linear when $(A,B)$ are fixed.
\end{lemma}
\begin{proof}
    Note that as $(\A,\B)$ come from a finite set, we can consider them as constants.
    Note that the first expression and the second are point-wise linear as we take $l_1$ norm. Thus, we have a finite number of linear regions, each a polytope.
    Next, note that we minimize a linear function in each linear region; thus, the minimum could be chosen to be at the region's defining points, as if the optimum is in the interior, on the boundary, the value is smaller.
    Thus, there exists a finite number of boundary points and we take minimum over them and a minimum of point-wise linear functions is point-wise linear.
\end{proof}


\ta{This is something we need to think carefully how to present. There is an underlying reason for the lack of upper-Lipschitzness, and it is that our metric becomes too coarse as the features grow in magnitude. We also need to say explicitly that the essential implication of this is that our embedding is \emph{better} than our metric. Then we can close this section  by saying that in the appendix we show that our embedding is bi-Lipschitz with respect to the TMD. }


==> text_backup_Sep_29/sec_numerical_experiments.tex <==
\section{Numerical Experiments}
\label{sec_numerical_experiments}
%
\nd{in the tables: our method is called SW, should be called FSW-GNN}

\ta{Our method name FSW-GNN is part of the paper title. No need to add "(Ours)" in my opinion}


Our experiments are divided into two categories: oversquashing and real-world benchmarks.
\paragraph{Over-squashing} Those tasks are taken from \cite{alon,bron}. 
Note that we are the first to show a solution to this problem, except for many methods adding virtual nodes as suggested in \cite{alon}. Adding a virtual node makes the radius two, thus skipping the over-squashing problem and not directly addressing it.
\cite{alon} constructed a tree graph with depth $r$, with $2^r$ nodes, and one of the leaves should propagate its label to the root. Note that this task is 1-WL solvable, and at least $r+1$ layers of MPNNs are needed. When $r$ is large, an exponential number of features are squashed into the root's node features, causing a potential over-squashing. \cite{alon} compared several MPNNs and showed that for large $r$ all models collapse. In our experiments, we took their implementation with a hidden dimension of $64$ for all models, searched for each of its best hyper-parameters, and reported the training accuracy. We checked for all radii between $2$ and $8$ and reported the findings in \ref{fig:Trees}. As can be seen, all models collapse at $r=8$ while we stay with the learning of $100\%$.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{tree.pdf}
    \caption{Trees models comparison.}
    \label{fig:Trees}
\end{figure}
Next, we took the three types of graphs from \cite{bron} with a problem radius of $r$ and $2r$ nodes with a complex topology that makes over-squashing more severe. \cite{bron} checked several MPNNs and showed all collapse at a radius of $15$ and some even before. We show our performance with the same hidden feature dimension and compare it with other models in \autoref{fig:comparison}, all baselines taken from \cite{bron}.
As can be seen, we are the only ones who succeed $100\%$ across all three graphs and radii. Our model begins to crack at around $20$ layers problem.
\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/cliquepath_plot.pdf}
        \caption{CliquePath task performance comparison}
        \label{fig:left}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ring_plot.pdf}
        \caption{Ring task performance comparison}
        \label{fig:middle}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/crossring_plot.pdf}
        \caption{CrossRing task performance comparison}
        \label{fig:right}
    \end{minipage}
    \caption{Comparison of models in all three learning tasks}
    \label{fig:comparison}
\end{figure}

\paragraph{Real world datasets}
For real-world benchmarks, we considered three types of datasets: LRGB \cite{lrgb2022}, MolHIV \cite{molhiv}, and node classification on single graph learning tasks taken from \cite{GCN+}.
\paragraph{LRGB and MolHIV}
We further evaluate our architectures on two larger datasets from LRGB \cite{lrgb2022}. The first, peptides-func, is a multi-label graph classification dataset. The second, peptides-struct, consists of the same graphs as peptides-func but with a regression task. Results in table \ref{tab:lrgb_datasets} show comparable results and in one-second place after \cite{davidson2024h}. Both experiments adhere to the 500K parameter constraint as in \cite{lrgb2022}. Regarding MolHIV, we report our results in \ref{auc_comparison} compared to other 1-WL equivalent methods. We report test errors in addition to validation errors, showing a possible data corruption.


\begin{table}[ht]
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Method} & \textbf{Test AUC} & \textbf{Validation AUC} \\
\hline
GIN & 0.7558 $\pm$ 0.0140 & \underline{0.8232 $\pm$ 0.0090} \\
GIN+FLAG & 0.7654 $\pm$ 0.0114 & 0.8225 $\pm$ 0.0155 \\
GCN & 0.7606 $\pm$ 0.0097 & 0.8204 $\pm$ 0.0141 \\
GCN+FLAG & \underline{0.7683 $\pm$ 0.0102} & 0.8176 $\pm$ 0.0087 \\
GCN+GraphNorm & \textbf{0.7883 $\pm$ 0.0100} & 0.7904 $\pm$ 0.0115 \\
FSW-GNN & 0.76666 $\pm$ 0.01591 & \textbf{0.82542 $\pm$ 0.00821} \\
\hline
\end{tabular}
\caption{Comparison of Methods based on Test and Validation AUC (mean ± std)}
\label{auc_comparison}
\end{table}



\paragraph{Single graph learning}
In the single graph learning, we compared to 1-WL equivalent methods that don't omit edges or nodes to compare only the aggregation impact and lack of invariance and having separation power stronger than WL. We compare our performance to several known methods in \autoref{tab:performance_comparison}. As we can see, we surpass in most of the tasks.
\begin{figure}[ht]
\centering
\scalebox{0.77}{
    \setlength{\tabcolsep}{3pt} %
    \begin{tabular}{l | cc}
        \hline
        Dataset & peptides-func (AP$\uparrow$) & peptides-struct (MAE$\downarrow$) \\ \hline
        GINE \cite{Hu*2020Strategies} & 0.6621$\pm$0.0067 & \underline{0.2473$\pm$0.0017} \\
        GCN \cite{kipf2017semisupervised} & 0.6860$\pm$0.0050 & \textbf{0.2460$\pm$0.0007} \\
        GatedGCN \cite{bresson2018residual} & 0.6765$\pm$0.0047 & 0.2477$\pm$0.0009 \\
        SortMPNN \cite{davidson2024h} & \textbf{0.6914$\pm$0.0056} & 0.2494$\pm$0.0021 \\
        FSW-GNN (ours) & \underline{0.6864$\pm$0.0048} & 0.2489$\pm$0.00155 \\ \hline
        Best model in universe & 0.73 & 0.242 \\ \hline
    \end{tabular}
}
\caption{LRGB results. Best in bold. Second best in \underline{underline}.}
\label{tab:lrgb_datasets}
\end{figure}
\begin{table}[ht]
    \centering
    \begin{tabular}{lccccccccc}
        \toprule
        Model      & Cora  & Cite. & Pubm. & Cham. & Squi. & Actor & Corn. & Texa. & Wisc. \\
        \midrule
        GCN        & 85.77 & 73.68 & \underline{88.13} & 28.18 & 23.96 & 26.86 & 52.70 & 52.16 & 45.88 \\
        GAT        & \textbf{86.37} & 74.32 & \underline{87.62} & 42.93 & 30.03 & 28.45 & 54.32 & 58.38 & 49.41 \\
        FSW-GNN & \underline{85.92}  & \textbf{75.24} &  87.5  & \textbf{50.79} &   \textbf{36.26}  & \textbf{33.6} & \textbf{72.43}  & \textbf{74.59} & \textbf{81.76}  \\
        \bottomrule
    \end{tabular}
    \caption{Performance comparison across different datasets and models, with SW as an additional method.}
    \label{tab:performance_comparison}
\end{table}

\begin{figure}[h!]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        width=10cm, height=8cm,
        xlabel={Number of MPNN layers},
        ylabel={Dirichlet Energy},
        grid=major,
        legend pos=north east
    ]
    
    % GCN data (blue)
    \addplot[
        color=blue,
        mark=o,
        thick
        ] coordinates {
        (2, 0.014372359961271286) (3, 0.0030192360281944275) (4, 0.0028000101447105408)
        (5, 0.003726869821548462) (6, 0.0029839787166565657) (7, 0.014826628379523754)
        (8, 0.011899886652827263) (9, 0.006362812593579292) (10, 0.011052481830120087)
        (11, 0.008961042389273643) (12, 0.004953503143042326) (13, 0.0016180472448468208)
        (14, 0.0004250822530593723) (15, 0.0031218724325299263)
    };
    \addlegendentry{GCN}

    % SW data (red)
    \addplot[
        color=red,
        mark=o,
        thick
        ] coordinates {
        (2, 0.23129764199256897) (3, 0.23935042321681976) (4, 0.23166564106941223)
        (5, 0.13226620852947235) (6, 0.17521896958351135) (7, 0.20060640573501587)
        (8, 0.11060592532157898) (9, 0.14070278406143188) (10, 0.1083298921585083)
        (11, 0.14121130108833313) (12, 0.08560832589864731) (13, 0.08076081424951553)
        (14, 0.0725787878036499) (15, 0.11434303969144821)
    };
    \addlegendentry{FSW-GNN}

    % GIN data (green)
    \addplot[
        color=green,
        mark=o,
        thick
        ] coordinates {
        (2, 0.14374399185180664) (3, 0.06146542355418205) (4, 0.06514272838830948)
        (5, 0.07730692625045776) (6, 0.06980648636817932) (7, 0.042782582342624664)
        (8, 0.054520830512046814) (9, 0.06063096597790718) (10, 0.06187702342867851)
        (11, 0.07470754534006119) (12, 0.046040840446949005) (13, 0.06190402805805206)
        (14, 0.028425956144928932) (15, 0.005265673156827688)
    };
    \addlegendentry{GIN}

    % GAT data (purple)
    \addplot[
        color=purple,
        mark=o,
        thick
        ] coordinates {
        (2, 0.0060063861310482025) (3, 0.008142106235027313) (4, 0.0010313894599676132)
        (5, 0.0012531251413747668) (6, 0.008989023976027966) (7, 0.0015892249066382647)
        (8, 0.0066517312079668045) (9, 0.0055049508810043335) (10, 0.007288204040378332)
        (11, 0.0064691416919231415) (12, 0.005511886905878782) (13, 0.003485677530989051)
        (14, 0.0036903168074786663) (15, 0.003497597761452198)
    };
    \addlegendentry{GAT}

    % GRAPH-SAGE data (cyan)
    \addplot[
        color=cyan,
        mark=o,
        thick
        ] coordinates {
        (2, 0.25541749596595764) (3, 0.18445533514022827) (4, 0.0262012779712677)
        (5, 0.3350397050380707) (6, 0.05011697858572006) (7, 0.47859227657318115)
        (8, 0.3238331973552704) (9, 0.45418787002563477) (10, 0.001550318324007094)
        (11, 0.0034304384607821703) (12, 0.005483350716531277) (13, 0.0014853696338832378)
        (14, 1.033821354212705e-05) (15, 0.0002989441272802651)
    };
    \addlegendentry{GRAPH-SAGE}

    \end{axis}
    \end{tikzpicture}
    \caption{Dirichlet Energy vs. Number of MPNN layers for various models on the Ring long-range task}
\end{figure}



==> text_backup_Sep_29/sec_problem_setting.tex <==
\section{Problem Setting}
\label{sec_problem_setting}
%
In this section we outline the problem setting, first providing the theoretical background of the problem, and then stating our objectives.

\paragraph{Vertex-featured graphs}
%
Our main objects of study are graphs with vertex features, represented as triplets $G=\br{V,E,X}$, where $V=\brc{v_i}_{i=1}^n$ is the set of vertices, $E\subseteq \setst{ \brc{v_i,v_j}}{i,j\in\brs{n}}$ is the set of undirected edges in $G$, and $X=\brs{\bx_1,\ldots,\bx_n}$ is a matrix containing the vertex feature vectors $\bx_i\in\Omega$, with $\Omega \subseteq \RR^d$ being the \emph{feature domain}. We denote by $\GNof\Omega$ the set of all vertex-featured graphs with at most $N$ vertices and corresponding features in $\Omega$. Throughout the paper we use $\brc{}$ to denote multisets.
%

\ta{Say somewhere that our theory can straightforwardly accommodate edge features and explain how.}
%

\ta{Maybe say something about the graph isomorphism problem before introducing the WL test.}


\paragraph{Weisfeiler-Leman test}
%
The Weisfeiler-Leman (WL) graph isomorphism test is designed to determine whether two graphs are \emph{isomorphic}, meaning they are identical up to relabeling their nodes. The test either concludes that the graphs are non-isomorphic or returns an indeterminate outcome. Given $G=\br{V,E,X}$, the test follows the recursive formula
%
\begin{equation}\label{eqdef_wl}
\begin{split}
    c^{0}_{v} \eqdefx & \X_{v}, \quad v \in V, 
    %
    \\ c^{t}_{v} \eqdefx & \textup{Combine}\br{c^{t-1}_{v},\textup{Aggregate}\br{\setst{c^{t-1}_{u}}{u \in \N_{v}}}},
    \quad
    1 \leq t \leq T,
    %
    \\ c^{T}_G \eqdefx & \textup{Readout}\br{\brc{c^{T}_{v_{1}},\ldots,c^{T}_{v_{n}}}},
\end{split}
\end{equation}
%
where Aggregate and Readout are functions that injectively map multisets of vectors in Euclidean space into another Euclidean space, Combine is an injective function from one Euclidean space to another, and $\N_{v}$ denotes the neighborhood of the vertex $v$ in $G$. 

\begin{definition*}[WL graph equivalence]
Two vertex-featured graphs $G$ and $\tilde{G}$ are said to be \emph{WL-equivalent}, denoted by $G \wleq \tilde G$, if $c^T_G = c^T_{\tilde G}$ for all $T \geq 0$. Otherwise, they are said to be \emph{WL-separable} or \emph{WL-distinguishable}.
\end{definition*}
%

It is a known fact \citep{grohe2021logic,morris2023weisfeiler} that for $G,\tilde G \in \GNd$, if the equality $c^T_G = c^T_{\tilde G}$ is satisfied for $T=N$, then it is satisfied for all $T \geq 0$, and thus $G \wleq \tilde G$.

While the WL test can distinguish most pairs of non-isomorphic graphs, there exist examples of non-isomorphic graph pairs that WL cannot separate; see \citep{fail_example}.
%
Note that there exist higher-order versions of this test called $k$-WL, $k \geq 2$, but in this paper, we consider only the $1$-WL test, denoted by WL for brevity.


\paragraph{Functions on graphs}
%
A \emph{graph function} is a function $F:\GNd\to\RR^m$ that maps vertex-featured graphs into a Euclidean space. The output of a graph function should depend only on the structure of the input graph and its vertex features; specifically, it should be invariant to permuting the vertex indices. 

\begin{definition*}[WL separation]
    A graph function $F:\GNof\Omega\to\RR^m$ is said to be \emph{WL-separating} if for any pair $G,\tilde G \in \GNof\Omega$, $G \wlneq \tilde G$ implies $F\of{G} \neq F\of{\tilde G}$. If the converse also holds, then $F$ is said to be \emph{WL-equivalent}.
\end{definition*}

\paragraph{Graph embeddings}
Any WL-equivalent graph function can be regarded as injective when defined on the \emph{quotient space} of $\GNof\Omega$ with respect to WL equivalence. We denote that space by $\GNofWL\Omega$. Thus, such function provides an \emph{embedding} of $\GNofWL\Omega$ into the Euclidean space $\RR^m$.  

Euclidean embeddings are an essential tool in machine learning on non-Euclidean data, such as graphs. 
%These embeddings map inputs from the non-Euclidean data domain, in our case $\GNd$, into a Euclidean space. By doing so, 
They enable the application of multi-layer perceptrons (MLPs) and other standard machine learning techniques to the embedded space instead of the original non-Euclidean space.

Ideally, we would desire an embedding that produces different outputs for every pair of non-isomorphic graphs, namely an injective function from $\GNd$ to $\RR^m$. However, such an embedding would provide a solution to the graph isomorphism problem, to which no polynomial-time solution has been found to date. A reasonable compromise is an embedding that produces different outputs for pairs of graphs distinguishable by WL. %This motivates the following definition.



\paragraph{Message passing neural networks}
%
Message Passing Neural Networks (MPNNs) are the most common neural architectures designed to compute graph functions. They operate on a similar principle to the WL test, but with the purpose of performing predictions on graphs rather than determining if they are isomorphic. 

Their core mechanism is the message-passing procedure, which maintains a hidden feature for each vertex and iteratively updates it as a function of the neighbor's features.
%
This process is outlined as follows:
%
\begin{enumerate}
    \item \textbf{Initialization: } The hidden feature $\bh^{0}_v$ of each node is initialized by its input feature $\bx_v$.
    %
    \item \textbf{Message aggregation:} Each node $v\in V$ aggregates messages from its neighbors by
    %
    \begin{equation}
        m_v^{\br{t}} \eqdef \textup{Aggregate}\of{ \setst{ \phi\of{\bh^{\br{t-1}}_u} } {u \in \N_v} } 
    \end{equation}
    %
    with $\phi$ referred to as a \emph{message function}, and Aggregate is a multiset function.
    %
    \item \textbf{Update step:} Each node updates its own hidden feature according to its aggregated messages and its previous hidden feature:
    %
    \begin{equation}
        \bh^{\br{t}}_v \eqdef \psi\of{ m_v^{\br{t}}, \bh^{\br{t-1}}_v },
    \end{equation}
    %
    with $\psi$ referred to as an \emph{update function}.
    %
    \item \textbf{Readout:} After $T$ iterations of steps 2-3, a global graph-level feature $\bh_G$ is computed from the multiset of hidden features 
    $\setst{ h^{\br{T}}_v}{v\in V}$ 
    by a \emph{readout function}:
    \begin{equation*}
        \bh_G \eqdef \textup{Readout}\of{\setst{ h^{\br{T}}_v}{v\in V}}.
    \end{equation*}
\end{enumerate}
%
Numerous MPNNs were proposed in recent years \citep{gin,Gilmer2017NeuralMP}\ta{cite more examples}, with the main difference between them being the specific choices of the message, aggregation, update and readout functions. 


There is a close connection between MPNNs and the WL test, as it was shown by \citet{xu2018how,morris2019WL} that the expressive power of MPNNs is upper-bounded by that of WL. Namely, if the WL test does not distinguish between two graphs $G$, $\tilde G$, then any MPNN is guaranteed to produce the same output (as well as all intermediate values) on $G$ and $\tilde G$. Conversely, if all functions used in an MPNN are injective, then the graph function it computes is WL-equivalent.
\ta{Cite examples of WL-separating MPNNs}
Examples of such MPNNs are summation-based \cite{amir2023neural} etc.


\nd{suggestion: this should be after discussion of injectivity and why it is not enough. We therefore need a notion of a 'natural metric' on graphs. Here are two suggestions for such metrics...}


\paragraph{WL-equivalent metric for graphs}
%
While the WL test determines whether two graphs are WL-equivalent, in our setting, we consider graphs with continuous features. Therefore, a method that quantifies the \emph{extent} to which two graphs are not WL-equivalent would be a more appropriate tool. This motivates the following definition.
%
\begin{definition*}[WL-equivalent metric]
    A \emph{WL-equivalent metric on $\GNd$} is a function $\rho:\GNd \times \GNd \to \RR_{\geq 0}$ that satisfies the following conditions for all $G_1, G_2, G_3 \in \GNd$:
    \begin{subequations}
    \begin{align}        
        \rho\of{G_1, G_2} &\eqx \rho\of{G_2, G_1}
        & \quad &\textup{\emph{Symmetry} }
        %
        \\ \rho\of{G_1, G_3} &\leqx \rho\of{G_1, G_2} + \rho\of{G_2, G_3}
        & \quad &\textup{\emph{Triangle inequality} }
        %
        \\ \rho\of{G_1, G_2} &= 0 \Longleftrightarrow G_1 \wleq G_2.
        & \quad &\textup{\emph{WL equivalence} }
    \end{align}
    \end{subequations}
\end{definition*}
%
Note that strictly speaking, such $\rho$ is a \emph{pseudometric} on $\GNd$ rather than a metric, as it allows distinct graphs to have a distance of zero if they are WL-equivalent. However, for convenience, we will use the term \emph{metric} to denote a pseudometric.

%Note that the above definition depends on the parameter $N$.


\paragraph{Tree Mover's Distance}
%
We now describe a WL-equivalent metric for vertex-featured graphs proposed by \citet{TMD}. This metric, named the Tree Mover's Distance (TMD), is based on building computation trees that simulate the WL procedure, and calculating distances between sub-trees using optimal transport. With the full definition given in \ta{the next section / in the appendix}, the TMD, denoted by $\TMD[L]\of{G,\tilde G}$ depends on a depth parameter $L$. The authors proved that under some assumptions, for two graphs $G_1$, $G_2$, $\TMD[L+1]\of{G_1,G_2}>0$ if and only if $G_1$ and $G_2$ are distinguishable by $L$ iterations of WL.
%
% a tree distance between the WL computation trees parameterized by $L \in \NN$, which can be
% written recursively as the sum of the distance between tree roots $r$ and the distance
% between the sub-trees rooting at r’s children.
% By construction $TMD$ holds the following properties:
% \begin{enumerate}
%     \item $WL^{L}(\G) = WL^{L}(\H) \iff TMD^{L+1}(\G,\H) = 0$
%     \item Homogeneity with respect to multiplication of the node features by a scalar.
% \end{enumerate}
%
Note that this implies that for $L = N+1$, $\TMD[L]\of{\argdot,\argdot}$ is a WL-equivalent metric on $\GNd$.

%As mentioned above, the TMD is computed by recursion on computation trees that simulate the WL test. At the depth required for TMD to achieve WL-equivalence on $\GNd$, its worst-case computational complexity is $\mathcal{O}\of{N^5\log N}$. Our first main objective in this paper is to introduce a simpler metric, which can be computed by solving a linear program in $\mathcal{O}\of{\argdot}$ time \ta{complete this}. \nd{overkill. This is an extremely well known metric discussed in several very related work. See references I sent in the chat. We have the rather minor goal of extending it to features. This would seem straightforward to poeple familiar with the problem.}



\paragraph{Bi-Lipschitzness}
%
The main weakness of the notion of separation is that it does not provide any information about the \emph{quality} of the separation. Without further assumptions, a WL-separating function may map two input graphs that are far apart in a metric sense to outputs that are very close, or even numerically indistinguishable, in the output Euclidean space.
%
To produce numerically robust embeddings, one would expect an embedding function $\emb$ to map graphs that are far apart in the original space $\GNof\Omega$ to vectors that are similarly far apart in the embedding space, and vice versa. The most common mathematical property used to describe this behavior is \emph{bi-Lipschitzness}.
%
\begin{definition*}[bi-Lipschitz embedding]
    Let $\rho$ be a WL-equivalent metric on $\GNof\Omega$. An embedding $\emb:\GNof\Omega\to\RR^m$ is said to be \emph{bi-Lipschitz with respect to $\rho$ on $\GNof\Omega$} if there exist constants $0<c\leq C < \infty$ such that
    \begin{equation}\label{eqdef_bilip}
        c \cdot \rho\of{G_1,G_2}
        \leq \norm{\emb\of{G_1}-\emb\of{G_1}}
        \leq C \cdot \rho\of{G_1,G_2}
    \end{equation}
    for any $G_1, G_2 \in \GNof\Omega$.
    
    If $\emb$ satisfies just the left- or right-hand side of \cref{eqdef_bilip}, it is said to be \emph{lower-Lipschitz} or \emph{upper-Lipschitz}, respectively, with respect to $\rho$ on $\GNof\Omega$.
\end{definition*}
%
In \cref{eqdef_bilip} and throughout our paper, a norm $\norm{\argdot}$ without an order denotes the $\ell_2$ norm.

Bi-Lipschitzness essentially ensures that the embedding approximately preserves the original distances in the input space $\GNof\Omega$, with the ratio $\tfrac{C}{c}$ providing an upper bound on the distortion induced by the embedding, akin to the condition number of a matrix. A low-distortion embedding enables using metric-based learning methods such as nearest-neighbor search and data clustering in the embedding space instead of in the original space, where calculating pairwise metrics are typically significantly more computationally intensive.

Our second main objective is thus to develop an embedding for vertex-featured graphs that is bi-Lipschitz and can be computed efficiently in practice.


%Note that some embedding could be Bi-Lipschitz with respect to one metric but not with respect to another.

\paragraph{Oversmoothing and oversquashing}
aa\ta{Consider introducing these phenomena here and argue that the root underlying cause for the two of them is the lack of bi-Lipschitzness. Alternatively, introduce them in the next section, as an addition after stating the properties of our embedding.}
\nd{should I try to write something?}

To summarize our objectives, we want to (1) derive a WL-equivalent metric that is simple and easy to compute, and (2) develop a bi-Lipschitz embedding with respect to this metric that can be computed easily in practice.
%
We conjecture that such an embedding may help address the root cause of over-squashing. This will be confirmed by our experiments.



==> text_backup_Sep_29/subsec_related_works.tex <==
\subsection{Related Works}
\label{subsec_related_works}
%
\ta{Question to Nadav: Where is the optimal place to introduce oversquashing?}

\nd{all current related work has already been cited, and can be deleted. Things that are relevant are MPNN that used sorting or reference distributions, discussion of bilipschitzness for graphs in the literatures. Other mentions of bilipscitnzess. }

\ta{Move the two following paragraphs to the introduction or merge them into \cref{subsec_theoretical_background}. This subsection should contain methods that we have to cite but are not an integral part of the story.} \tared{Reminder}
%
\paragraph{graph isomorphism tests and GNNs}
As graph isomorphism is conjectured to be a hard problem, several graph isomorphism tests have been studied. The most famous is the WL test. In this test, the initial coloring of a node is its node feature, and the color is refined according to its color and neighbor's color. This test separates most graphs but not all \cite{fail_example}. A higher order of K-WL was introduced to separate more graphs, and it's known that (k+1)-WL can separate more graphs than K-WL but not all. \cite{Gilmer2017NeuralMP} showed that many methods fall under the message-passing neural networks framework. \cite{xu2018how,morris2019WL}, showed the 1-WL test bounds the expressiveness power of MPNNs. Thus, any two graphs 1-WL can't distinguish any MPNN will output the same embedding.
\paragraph{Graph Metrics}
Measuring distance between graphs is a topic in graph theory. A naive approach could be minimization over all permutations, but it's intractable. \cite{TMD} presented a distance equivalent to 1-WL and could be computed in a polynomial time.


==> text_copy/sec_conclusion.tex <==
\section{Conclusion}
\label{sec_conclusion}
%
In conclusion, ...

==> text_copy/sec_introduction.tex <==
\section{introduction}
\label{sec_introduction}
%


Graph neural networks are a central research topic in contemporary machine learning research, with a multitude of different models being proposed. Many of the most popular models, such as GraphSage \cite{XXX}, GAT \cite{XXX}, and GCN \cite{XXX}, can be seen as an instantiation of Message Passing Neural Networks (MPNNs) \cite{Gilmer2017NeuralMP}. 

A well known limitation of MPNNs is that they cannot differentiate between all distinct graphs. In fact, a pair of distinct graphs which cannot be separated by the Weisfeiler-Lehman (WL) graph isomorphism test will not be separated by \emph{any} MPNN  \cite{xu2018how}. Conversely, it is shown in \cite{xu2018how,morris2019WL} that suitably chosen MPNN will be able to separate all pairs of graphs which are separable by WL. We will say that such an MPNN is WL-equivalent. 

Recent work had shown that WL-equivalent MPNN can be unrealistically small \cite{amir2023neural,XXX}. For these MPNN, it was observed that the separation of graphs is so  weak that extra precision digits are needed to observe it \nd{(see XXXanalytic,snir)}. Furthermore, MPNN often suffer from  oversmoothing \nd{cite}, where  distinct nodes are assigned near-identical node features.  These two observations motivate the development of \emph{quantitative} estimate of MPNN separation, by means of 
bi-Lipschitz stability guarantees. These guarantees would ensure that  euclidean distances in the MPNN feature space are neither much larger nor much smaller than distances in the original graph-space, which are defined by a suitable graph-metric (defined up to WL equivalence).

The notion of 
Bi-Lipschitz stability analysis is common in various fields \cite{XXX}, and has been recently become a topic of interest in the GNN community as well. Indeed, a recent survey \cite{XXX} identified bi-Lipschitz guarantees for MPNNs as a key challenge for future GNN research. 

Some first steps towards addressing these challenges have already been made. It has been observed in \cite{XXXjegelka,XXXyair} that many MPNN models are upper-Lipscitz. However, essentially all popular MPNN models, such as those based on sum-pooling, are not lower-Lipschitz continuous \cite{davidson2024h}. In contrast, \cite{davidson2024h} propose a new MPNN, based on sorting-based aggregations from \cite{balan2022permutation}, which \emph{is} bi-Lipschitz \emph{in expectation}, a weaker notion than the standard bi-Lipschitz definition. 

\nd{In this paper... stopped here}  






\nd{I will continue working on intro and related work on Sunday. Also will add the missing citations}
% Motivated by  applications for chemoinformatics \cite{Gilmer2017NeuralMP}, social networks \cite{borisyuk2024lignn},
% and recommendation systems \cite{gao2023survey}, and more, permutation invariant deep learning for 
% graphs has gained increasing interest in recent years. This, in turn, has inspired several theoretical
% works that analyze common GNNs and their expressive power and limitations.
%  Our focus in this paper will be on Message Passing Neural Network (MPNN) \cite{Gilmer2017NeuralMP} paradigm, which includes a variety of popular GNNs \cite{xu2018how, Gilmer2017NeuralMP, kipf2017semisupervised}. In their seminal works, \cite{xu2018how, morris2019WL} prove that MPNNs are at most expressiveness as the Weisfeiler-Lehman (WL) graph isomorphism test \cite{weisfeiler1968reduction}.
% Accordingly, maximally expressive MPNNs are those that can separate all graph pairs that
% are WL-separable. \cite{xu2018how, morris2019WL} shows that MPNNs that employ injective multi-set functions are maximally expressive. Examples of MPNNs that are 1-WL equivalent are \cite{gin}.
% However, while current theory ensures separation, it tells us little about the separation quality, so that embeddings of "separable" objects may
% be highly similar, to the extent that in some cases, graphs that can be theoretically separated by
% maximally expressive MPNNs are completely identical on a computer with fixed finite precision (see
% \cite{bravo2024dimensionality}, figure 1). To study the separation quality of permutation invariant models, we will search for bi-lifshiz continuity guarantees. \cite{amir2023neural} showed summation-based aggregation functions are not bi-lifshiz with respect to the distance between multi-sets;\ta{We actually did it in \citep{amir2023neural}} thus, all summation-based GNNs are not bi-lifshiz. Recently \cite{davidson2024h} presented a network that is a bi-lifhsiz on expectation over weights drawn uniformly from the circle. In this work, we show a Bi-lifshiz embedding on any compact domain(not in expectation) with respect to a metric equivalent to 1-WL.

% We demonstrate our theoretical superiority on long-range tasks like LRGB \cite{lrgb2022}, short-range tasks like Cora \cite{cora}, and over-squashing tasks taken from \cite{alon, bron} without global nodes.

\inputtext{subsec_related_works}

==> text_copy/sec_main_contributions.tex <==
\section{Main Contributions}
\label{sec_main_contributions}
%
In this section, we outline our main contributions. First we describe our proposed metric for vertex-featured graphs. Then we present our bi-Lipschitz GNN, and discuss its theoretical properties.
%

%\subsection{WL-equivalent metric for vertex-featured graphs}
%\label{subsec_metric}
%
We start by describing our proposed metric and then show that it is equivalent to the WL test for vertex-featured graphs.
%
Our metric is inspired by the work of \citet{book}, who defined a metric for featureless graphs with a fixed number of vertices. Let $G$ and $\tilde G$ be two graphs, each with $n$ vertices, and let their corresponding adjacency matrices be $A$ and $\tilde A$. Their metric is defined as
%
\begin{equation}\label{eqdef_metric_ds_nofeat}
    \rho\of{G,\tilde G}
    =
    \min_{S\in\D_n} \ 
    \norm{AS-S\tilde A},
\end{equation}
%
where $\D_n$ is the space of all $n\times n$ doubly-stochastic matrices, and $\norm{\argdot}$ is an arbitrary operator norm. They also proved that this metric assigns zero distance to two graphs if and only if they are WL-indistinguishable.

Building on this idea, we adapt the above metric to vertex-featured graphs with varying numbers of vertices, by augmenting it as follows:
%
\begin{equation}\label{eqdef_metric_ds}
    \rhods\of{G,\tilde G}
    =
    \abs{n-\tilde n}
    +
    \min_{S\in\Pi\of{n,\tilde n}} \ 
    \norm{AS-S\tilde A}
    +
    \sum_{i\in\brs{n}, j\in\brs{\tilde n}} s_{ij}
    \norm{\bx_i-\btx_j},
\end{equation}
%
where: 
(1) $n=\abs{V}$, $\tilde n = \abs{\tilde V}$; (2) $\Pi\of{n,\tilde n}$ is the set of $n \times \tilde n$ matrices $S$ that satisfy $\sum_{j=1}^{\tilde n} S_{ij} = \tfrac{1}{n}$, $\sum_{i=1}^{n} S_{ij} = \tfrac{1}{\tilde n}$;
(3) $\bx_i$ and $\btx_j$ denote the vertex features of $G$ and $\tilde G$ respectively. The norms in \cref{eqdef_metric_ds} can be arbitrary. In the rest of this paper we use $\norm{\argdot}$ to denote the $\ell_2$ norm for vectors and entrywise $\ell_2$ norm for matrices.

%The following theorem states that $\rhods\of{\argdot,\argdot}$ is indeed a WL-equivalent metric. A proof is in the appendix.\ta{add reference}
%
\begin{theorem}[Proof in \cref{metric_property}]
    Let $\rhods: \GNd \times \GNd \to \RR_{\geq 0}$ be as in \cref{eqdef_metric_ds}.
    Then $\rhods$ is a WL-equivalent metric.
    %Let $G,\tilde G \in \GNd$. Then $\rhods\of{G,\tilde G} = 0$ if and only if $G \wleq \tilde G$.
\end{theorem}

\ta{Here maybe say something good about our metric. e.g.:}
The metric $\rhods$ provides a natural measure to quantify the difference between two graphs with vertex features. When taking the norms to be $\ell_1$ norms, it can be computed easily by a linear programming solver.

%\ta{State something like this when we're chosen the norm and we're sure of the complexity: }
%
%The metric $\rhods$ is defined by a linear program that can be solved in $\O\of{\argdot}$ time, which matches the complexity of the WL test. However, unlike WL, here the outcome not only determines whether two vertex-featured graphs are WL-equivalent or not, but also quantifies the extent to which they are inequivalent.


%\subsection{Bi-Lipschitz Embedding and Graph Neural Network}
%\label{subsec_bilipschitz_gnn}
%
We now present our main contribution: a novel MPNN with WL-equivalent separation power for vertex-featured graphs. Unlike other MPNNs in this class, this MPNN maps input graphs into the output Euclidean space in a bi-Lipschitz manner, both with respect to the metric $\rhods$ and the Tree Mover’s Distance. 

The core innovation in our MPNN lies in its message aggregation method. As discussed in \cref{sec_problem_setting}, most prevalent MPNNs aggregate messages using simple pooling operations such as sum- or max-pooling. However, theoretical analyses in recent years have revealed significant limitations in these methods. \citet{amir2023neural} showed that sum-pooling inevitably induces infinite distortion on its input space, thereby making bi-Lipschitzness impossible; see also \citep{cahill2023bilipschitz} for a related result.\ta{Is this the proper way to cite Cahill?} Furthermore, \citet{xu2018how} showed that max-pooling is not even injective, as it fails to account for repetitions of multiset elements. These findings suggest that traditional pooling methods may pose a substantial bottleneck in the performance of MPNNs.

More sophisticated pooling methods have been proposed in recent works.
%
\citet{davidson2024h} proposed an MPNN and proved that it is 2-Holder in expectation. Although they did not prove this in their paper, it can be shown that their MPNN is bi-Lipschitz. However, their pooling mechanism requires a priori knowledge of the highest possible vertex degree in the input graphs, which is a significant limitation. Other pooling mechanisms were proposed in \citet{fspool,naderializadeh2021pooling}, but their methods do not have bi-Lipschitzness guarantees. \ta{Cite Balan? He did not discuss MPNNs in his work. e.g. Similarly, a pooling method based on sorting was proposed by Balan et al., but it only accommodates multisets of fixed size, and thus is only applicable to regular graphs.}

%\ta{Cite Yair's work and other works that used bi-Lipschitz embeddings (Kolouri? FSpool? Balan?)} \nd{indeed. Especially Yair. Need to explain similarities and differences. I would emphasize the issue of varying cardinalities. Also mention  'in expectation' but say yair also is probably bi-lipschitz in the standard sense, he just didn't prove it.}


To address these limitations, we build on the recent work of \citet{amir2024injective}, who proposed the \emph{Fourier Sliced-Wasserstein (FSW) embedding} for multisets. In a nutshell, this embedding operates by taking random one-dimensional projections (called \emph{slices}) of the input multiset, calculating the quantile function for each slice, and sampling its Fourier transform at a random frequency. Importantly, they proved that this embedding is bi-Lipschitz with respect to the Wasserstein distance. This property ensures better numerical retention of information, making the FSW embedding a potentially superior candidate for multiset aggregation. Our proposed architecture, which we name \textbf{FSW-GNN}, leverages the FSW embedding as its message aggregation mechanism. We now provide a formal description. 

The FSW embedding $\embfsw\of{\argdot}$ takes input multisets over $\RR^d$ and maps them into a Euclidean space $\RR^m$. It depends on parameters that are drawn randomly from a specific distribution; see \citep{amir2024injective} for more details. It was shown that with a sufficiently large $m$, with probability 1 the resulting embedding is bi-Lipschitz with respect to the Wasserstein distance.

The FSW-GNN processes input graphs $G=\br{V,E,X}$ by $T$ message-passing iterations according to the following recursive formula:
%
\begin{equation}\label{eqdef_fswgnn}
\begin{split}
    \bh^{\br{0}}_{v} \eqdefx & \bx_{v},
    %\quad v \in V, 
    %
    \\ \bq_v^{\br{t}} 
    \eqdefx &
    \embfswt[t]\of{ \setst{ \bh^{\br{t-1}}_u } {u \in \N_v} }, 
    \quad 1 \leq t \leq T
    \\ \bh^{\br{t}}_v
    \eqdefx &
    \Phi^{\br{t}} \of{ \brs{\bh^{\br{t-1}}_v;\bq^{\br{t}}_v}},
\end{split}
\end{equation}
%
where the functions $\embfswt[t]$ are all instances of the FSW embedding,
% with output dimension $m$, to be determined later;
% $\bM^{\br{t}}$ are matrices with random \nd{learned}\ta{not in the embedding} coefficients, all of whose output dimension is $m$;
% 
$\Phi^{\br{t}}$ are MLPs,
and $\brs{\bx; \by}$ denotes column-wise concatenation of column vectors $\bx$ and $\by$. Finally, a graph-level output is computed by:
%
\begin{equation}\label{eqdef_fswgnn_readout}
    \bh_G \eqdef 
    \Psi \circ
    \embfswglob\of{\setst{ \bh^{\br{T}}_v}{v\in V}},
\end{equation}
%
where, again, $\embfswglob$ is an FSW embedding, and $\Psi$ is an MLP.

The following \lcnamecref{thm_fswgnn_is_wl_equivalent} shows that with the appropriate choice of MLP sizes and number of iterations $T$, our proposed architecture has the separation power of the WL test.
%
\begin{theorem}\label{thm_fswgnn_is_wl_equivalent}
    %Consider the space of vertex-featured graphs $\GNof\Omega$ over the feature domain $\Omega\subset\RR^d$, and suppose that $\Omega$ is compact.
    Consider the FSW-GNN architecture defined in \cref{eqdef_fswgnn,eqdef_fswgnn_readout} for input graphs in $\GNd$, with $T=N$ iterations, all MLPs being one-layer matrices with output dimension $m \geq 2Nd+2$ and no activation, and all FSW embeddings having output dimension $m$. Suppose all FSW embeddings are initialized independently at random, and all MLPs have random entries drawn from an absolutely-continuous distribution over $\RR$. 
    Then with probability 1, the following holds: For any pair of graphs $G, \tilde G \in \GNd$, the corresponding outputs $\bh_G$ and $\bh_{\tilde G}$ computed by the FSW-GNN are equal if and only if $G \wleq \tilde G$.
\end{theorem}
%
%The probability in \cref{thm_fswgnn_is_wl_equivalent} is over the matrices $\bM^{\br{t}}$ and embedding functions $\embfswt[t]$ and $\embfswglob$, which depend on random parameters. 
%Note that the theorem does not require all embedding functions to be generated independently. In fact, two instances suffice: one for $\embfswt[1]$, which maps input multisets in $\RR^d$ into a single vector in $\RR^m$, and another instance for all $\embfswt[t]$ with $2 \leq t \leq T$ and for $\embfswglob$, all of which map input multisets in $\RR^m$ into a single vector in $\RR^m$.

The proof of \cref{thm_fswgnn_is_wl_equivalent} is based on the study of $\sigma$-subanalytic functions and the \emph{Finite Witness Theorem}, introduced in \citep{amir2023neural}.

It is worth noting that the output dimension $m$ required in practice is typically considerably lower than the one required in \cref{thm_fswgnn_is_wl_equivalent}. This can be explained by the following fact: If all input graphs come from a sub-manifold of $\GNd$ with intrinsic dimension $D$ significantly lower than the ambient dimension $n\cdot d$, then it can be shown that $m=2D+2$ suffices for WL-equivalence.


\paragraph{From separation to bi-Lipschitzness}
%
We now show that the WL-equivalence property of the FSW-GNN implies that it is in fact bi-Lipschitz, as stated in the following theorem.

\begin{theorem}\label{thm_fswgnn_is_bilip}
Let $\Omega \subset \RR^d$ be compact. Then under the assumptions of
\cref{thm_fswgnn_is_wl_equivalent}, the FSW-GNN is bi-Lipschitz with respect to $\rhods$ and TMD on $\GNof\Omega$.
\end{theorem}
\ta{A. Note that strictly speaking, the TMD part is true only if we augment all vertex feature vectors with a coordinate of 1. B. I skipped the part of bi-Lipschitzness without compactness assumption. This is too complex for the main text.} \nd{good}

We now give a high-level explanation of the proof idea. The full proof is in the appendix. \ta{verify}
%
To prove \cref{thm_fswgnn_is_bilip}, we rely on the following facts: (1) the output of FSW-GNN for an input graph $G=\br{V,E,X}$ is piecewise-linear with respect to the vertex-feature matrix $X$. This follows from properties of the FSW embedding functions used in \cref{eqdef_fswgnn,eqdef_fswgnn_readout}. (2) both metrics $\rhods$ and TMD can be transformed, with bounded distortion, into  piecewise-linear metrics by choosing all the vector norms they employ to be the $\ell_1$ norm. The claim them follows from these observations and the following \lcnamecref{thm_pwl_ratio_bound}:
%
\begin{lemma}
\label{thm_pwl_ratio_bound}
    Let $f,g: M \to \RR_{\geq 0}$ be non-negative piece-wise-linear functions defined on a compact polygon $M \subset \RR^d$. Suppose that for all $x\in M$, $f(x) = 0$ if and only if $g(x)=0$. Then there exist real constants $c,C > 0$ such that
    \begin{equation}\label{eq_pwl_functions_ratio_bound}
        c \cdot g\of{x} \leq f\of{x} \leq C \cdot g\of{x}
    \end{equation}
    for all $x \in M$ for which $g\of{x}>0$.
\end{lemma}

% The rest of the proof is as follows: Let $G,\tilde G \in \GNof\Omega$, $G=\br{V,E,X}$ and $\tilde G=\br{\tilde V, \tilde E, \tilde X}$, with $n$ and $\tilde n$ vertices respectively. It is enough to show that the bi-Lipschitz ratio is bounded on all choices of $X \in \Omega^n$, $\tilde X \in \Omega^{\tilde n}$, since there is a finite number of choices of $n,\tilde n \leq N$ and edges $E$, $\tilde E$. Define the function $f\of{X,\tilde X} = \norm{\bh_G - \bg_{\tilde G}}_1$, $g\of{X,\tilde X} = \rho\of{G,\tilde G}$, where $\rho$ is either $\rhods$ or TMD. By the comment above, both $f$ and $g$ are piecewise linear. Since both FSW-GNN and the metric $\rho$ are WL-equivlanet, $f$ and $g$ have the same zero set. Thus, \cref{thm_pwl_ratio_bound} guarantees the existence of Lipschitz constants $c,C$. Q.E.D.

\redline{End of Section}

\begin{lemma}
    Define $g(\G,\H) = d(\G,\H),f(\G,\H)=||\E(\G)-\E(\H)||$, where $g$ is some 1-WL equivalent piece-wise linear metric, and $\E$ to be a separating piece-wise linear embedding, then by the above lemma, the embedding is actually Bi-lifshiz on any compact set.
\end{lemma}
We need to find piece-wise linear embedding and metric to fulfill the lemma's conditions. Regarding the embedding, assume we have such embedding, and in the following sections, we detail the construction of such embedding denoted by $\E$. Regarding the metric, we now show this metric is indeed piece-wise linear
\ta{I'm not sure whether we need to state this formally in a lemma or not, but for sure we don't need to prove it in the main text.}
We now show that our embedding is \textbf{not} upper lifshiz with respect to $d_{S}$ on a non-bounded domain, but it's lower lifshiz even in the non-bounded domain.  Thus showing a limitation of our metric.
\ta{I wouldn't state in a lemma in the main text that our embedding is not upper lipschitz. I would just this briefly in one or two sentences somewhere at the end of the section, and perhaps refer the reader to further discussion in the appendix.}
\begin{lemma}
     Our embedding is \textbf{not} upper lifshiz with respect to $d_{S}$ on the non-bounded domain, but it's lower lifshiz even in the non-bounded domain.
\end{lemma}
\begin{proof}
 In the appendix we show a series of graphs with $4$ vertices $\{(\G_{n},\H_{n})\}$ such that $d_{S}(\G_{n},\H_{n})\leq 1$ but, $lim_{n\rightarrow \infty}||\E(\G_{n},\H_{n})||=\infty$.
\end{proof}
This example shows that even if the features go to infinity, the distance between graphs can be bounded. In the next metric that is homogenous, this phenomenon can't happen.
\ta{This is for me to write: }
A key component in our GNN 




\ta{It would be more efficient to simply state the main bi-Lipschitzness theorem in the next subsection, then add a short proof-idea paragraph that just says in words that both the embedding and metric are piecewise linear, and state \cref{thm_pwl_ratio_bound}. The full proof with actual lemmas about piecewise linearity is better deferred to the appendix.}
\begin{lemma}
    $d_{S}$ is piece-wise linear when $(A,B)$ are fixed.
\end{lemma}
\begin{proof}
    Note that as $(\A,\B)$ come from a finite set, we can consider them as constants.
    Note that the first expression and the second are point-wise linear as we take $l_1$ norm. Thus, we have a finite number of linear regions, each a polytope.
    Next, note that we minimize a linear function in each linear region; thus, the minimum could be chosen to be at the region's defining points, as if the optimum is in the interior, on the boundary, the value is smaller.
    Thus, there exists a finite number of boundary points and we take minimum over them and a minimum of point-wise linear functions is point-wise linear.
\end{proof}


\ta{This is something we need to think carefully how to present. There is an underlying reason for the lack of upper-Lipschitzness, and it is that our metric becomes too coarse as the features grow in magnitude. We also need to say explicitly that the essential implication of this is that our embedding is \emph{better} than our metric. Then we can close this section  by saying that in the appendix we show that our embedding is bi-Lipschitz with respect to the TMD. }


==> text_copy/sec_numerical_experiments.tex <==
\section{Numerical Experiments}
\label{sec_numerical_experiments}
%
\nd{in the tables: our method is called SW, should be called FSW-GNN}

\ta{Our method name FSW-GNN is part of the paper title. No need to add "(Ours)" in my opinion}


Our experiments are divided into two categories: oversquashing and real-world benchmarks.
\paragraph{Over-squashing} Those tasks are taken from \cite{alon,bron}. 
Note that we are the first to show a solution to this problem, except for many methods adding virtual nodes as suggested in \cite{alon}. Adding a virtual node makes the radius two, thus skipping the over-squashing problem and not directly addressing it.
\cite{alon} constructed a tree graph with depth $r$, with $2^r$ nodes, and one of the leaves should propagate its label to the root. Note that this task is 1-WL solvable, and at least $r+1$ layers of MPNNs are needed. When $r$ is large, an exponential number of features are squashed into the root's node features, causing a potential over-squashing. \cite{alon} compared several MPNNs and showed that for large $r$ all models collapse. In our experiments, we took their implementation with a hidden dimension of $64$ for all models, searched for each of its best hyper-parameters, and reported the training accuracy. We checked for all radii between $2$ and $8$ and reported the findings in \ref{fig:Trees}. As can be seen, all models collapse at $r=8$ while we stay with the learning of $100\%$.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{tree.pdf}
    \caption{Trees models comparison.}
    \label{fig:Trees}
\end{figure}
Next, we took the three types of graphs from \cite{bron} with a problem radius of $r$ and $2r$ nodes with a complex topology that makes over-squashing more severe. \cite{bron} checked several MPNNs and showed all collapse at a radius of $15$ and some even before. We show our performance with the same hidden feature dimension and compare it with other models in \autoref{fig:comparison}, all baselines taken from \cite{bron}.
As can be seen, we are the only ones who succeed $100\%$ across all three graphs and radii. Our model begins to crack at around $20$ layers problem.
\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/cliquepath_plot.pdf}
        \caption{CliquePath task performance comparison}
        \label{fig:left}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ring_plot.pdf}
        \caption{Ring task performance comparison}
        \label{fig:middle}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/crossring_plot.pdf}
        \caption{CrossRing task performance comparison}
        \label{fig:right}
    \end{minipage}
    \caption{Comparison of models in all three learning tasks}
    \label{fig:comparison}
\end{figure}

\paragraph{Real world datasets}
For real-world benchmarks, we considered three types of datasets: LRGB \cite{lrgb2022}, MolHIV \cite{molhiv}, and node classification on single graph learning tasks taken from \cite{GCN+}.
\paragraph{LRGB and MolHIV}
We further evaluate our architectures on two larger datasets from LRGB \cite{lrgb2022}. The first, peptides-func, is a multi-label graph classification dataset. The second, peptides-struct, consists of the same graphs as peptides-func but with a regression task. Results in table \ref{tab:lrgb_datasets} show comparable results and in one-second place after \cite{davidson2024h}. Both experiments adhere to the 500K parameter constraint as in \cite{lrgb2022}. Regarding MolHIV, we report our results in \ref{auc_comparison} compared to other 1-WL equivalent methods. We report test errors in addition to validation errors, showing a possible data corruption.


\begin{table}[ht]
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Method} & \textbf{Test AUC} & \textbf{Validation AUC} \\
\hline
GIN & 0.7558 $\pm$ 0.0140 & \underline{0.8232 $\pm$ 0.0090} \\
GIN+FLAG & 0.7654 $\pm$ 0.0114 & 0.8225 $\pm$ 0.0155 \\
GCN & 0.7606 $\pm$ 0.0097 & 0.8204 $\pm$ 0.0141 \\
GCN+FLAG & \underline{0.7683 $\pm$ 0.0102} & 0.8176 $\pm$ 0.0087 \\
GCN+GraphNorm & \textbf{0.7883 $\pm$ 0.0100} & 0.7904 $\pm$ 0.0115 \\
FSW-GNN & 0.76666 $\pm$ 0.01591 & \textbf{0.82542 $\pm$ 0.00821} \\
\hline
\end{tabular}
\caption{Comparison of Methods based on Test and Validation AUC (mean ± std)}
\label{auc_comparison}
\end{table}



\paragraph{Single graph learning}
In the single graph learning, we compared to 1-WL equivalent methods that don't omit edges or nodes to compare only the aggregation impact and lack of invariance and having separation power stronger than WL. We compare our performance to several known methods in \autoref{tab:performance_comparison}. As we can see, we surpass in most of the tasks.
\begin{figure}[ht]
\centering
\scalebox{0.77}{
    \setlength{\tabcolsep}{3pt} %
    \begin{tabular}{l | cc}
        \hline
        Dataset & peptides-func (AP$\uparrow$) & peptides-struct (MAE$\downarrow$) \\ \hline
        GINE \cite{Hu*2020Strategies} & 0.6621$\pm$0.0067 & \underline{0.2473$\pm$0.0017} \\
        GCN \cite{kipf2017semisupervised} & 0.6860$\pm$0.0050 & \textbf{0.2460$\pm$0.0007} \\
        GatedGCN \cite{bresson2018residual} & 0.6765$\pm$0.0047 & 0.2477$\pm$0.0009 \\
        SortMPNN \cite{davidson2024h} & \textbf{0.6914$\pm$0.0056} & 0.2494$\pm$0.0021 \\
        FSW-GNN (ours) & \underline{0.6864$\pm$0.0048} & 0.2489$\pm$0.00155 \\ \hline
        Best model in universe & 0.73 & 0.242 \\ \hline
    \end{tabular}
}
\caption{LRGB results. Best in bold. Second best in \underline{underline}.}
\label{tab:lrgb_datasets}
\end{figure}
\begin{table}[ht]
    \centering
    \begin{tabular}{lccccccccc}
        \toprule
        Model      & Cora  & Cite. & Pubm. & Cham. & Squi. & Actor & Corn. & Texa. & Wisc. \\
        \midrule
        GCN        & 85.77 & 73.68 & \underline{88.13} & 28.18 & 23.96 & 26.86 & 52.70 & 52.16 & 45.88 \\
        GAT        & \textbf{86.37} & 74.32 & \underline{87.62} & 42.93 & 30.03 & 28.45 & 54.32 & 58.38 & 49.41 \\
        FSW-GNN & \underline{85.92}  & \textbf{75.24} &  87.5  & \textbf{50.79} &   \textbf{36.26}  & \textbf{33.6} & \textbf{72.43}  & \textbf{74.59} & \textbf{81.76}  \\
        \bottomrule
    \end{tabular}
    \caption{Performance comparison across different datasets and models, with SW as an additional method.}
    \label{tab:performance_comparison}
\end{table}

\begin{figure}[h!]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        width=10cm, height=8cm,
        xlabel={Number of MPNN layers},
        ylabel={Dirichlet Energy},
        grid=major,
        legend pos=north east
    ]
    
    % GCN data (blue)
    \addplot[
        color=blue,
        mark=o,
        thick
        ] coordinates {
        (2, 0.014372359961271286) (3, 0.0030192360281944275) (4, 0.0028000101447105408)
        (5, 0.003726869821548462) (6, 0.0029839787166565657) (7, 0.014826628379523754)
        (8, 0.011899886652827263) (9, 0.006362812593579292) (10, 0.011052481830120087)
        (11, 0.008961042389273643) (12, 0.004953503143042326) (13, 0.0016180472448468208)
        (14, 0.0004250822530593723) (15, 0.0031218724325299263)
    };
    \addlegendentry{GCN}

    % SW data (red)
    \addplot[
        color=red,
        mark=o,
        thick
        ] coordinates {
        (2, 0.23129764199256897) (3, 0.23935042321681976) (4, 0.23166564106941223)
        (5, 0.13226620852947235) (6, 0.17521896958351135) (7, 0.20060640573501587)
        (8, 0.11060592532157898) (9, 0.14070278406143188) (10, 0.1083298921585083)
        (11, 0.14121130108833313) (12, 0.08560832589864731) (13, 0.08076081424951553)
        (14, 0.0725787878036499) (15, 0.11434303969144821)
    };
    \addlegendentry{FSW-GNN}

    % GIN data (green)
    \addplot[
        color=green,
        mark=o,
        thick
        ] coordinates {
        (2, 0.14374399185180664) (3, 0.06146542355418205) (4, 0.06514272838830948)
        (5, 0.07730692625045776) (6, 0.06980648636817932) (7, 0.042782582342624664)
        (8, 0.054520830512046814) (9, 0.06063096597790718) (10, 0.06187702342867851)
        (11, 0.07470754534006119) (12, 0.046040840446949005) (13, 0.06190402805805206)
        (14, 0.028425956144928932) (15, 0.005265673156827688)
    };
    \addlegendentry{GIN}

    % GAT data (purple)
    \addplot[
        color=purple,
        mark=o,
        thick
        ] coordinates {
        (2, 0.0060063861310482025) (3, 0.008142106235027313) (4, 0.0010313894599676132)
        (5, 0.0012531251413747668) (6, 0.008989023976027966) (7, 0.0015892249066382647)
        (8, 0.0066517312079668045) (9, 0.0055049508810043335) (10, 0.007288204040378332)
        (11, 0.0064691416919231415) (12, 0.005511886905878782) (13, 0.003485677530989051)
        (14, 0.0036903168074786663) (15, 0.003497597761452198)
    };
    \addlegendentry{GAT}

    % GRAPH-SAGE data (cyan)
    \addplot[
        color=cyan,
        mark=o,
        thick
        ] coordinates {
        (2, 0.25541749596595764) (3, 0.18445533514022827) (4, 0.0262012779712677)
        (5, 0.3350397050380707) (6, 0.05011697858572006) (7, 0.47859227657318115)
        (8, 0.3238331973552704) (9, 0.45418787002563477) (10, 0.001550318324007094)
        (11, 0.0034304384607821703) (12, 0.005483350716531277) (13, 0.0014853696338832378)
        (14, 1.033821354212705e-05) (15, 0.0002989441272802651)
    };
    \addlegendentry{GRAPH-SAGE}

    \end{axis}
    \end{tikzpicture}
    \caption{Dirichlet Energy vs. Number of MPNN layers for various models on the Ring long-range task}
\end{figure}



==> text_copy/sec_problem_setting.tex <==
\section{Problem Setting}
\label{sec_problem_setting}
%
In this section we outline the problem setting, first providing the theoretical background of the problem, and then stating our objectives.

\paragraph{Vertex-featured graphs}
%
Our main objects of study are graphs with vertex features, represented as triplets $G=\br{V,E,X}$, where $V=\brc{v_i}_{i=1}^n$ is the set of vertices, $E\subseteq \setst{ \brc{v_i,v_j}}{i,j\in\brs{n}}$ is the set of undirected edges in $G$, and $X=\brs{\bx_1,\ldots,\bx_n}$ is a matrix containing the vertex feature vectors $\bx_i\in\Omega$, with $\Omega \subseteq \RR^d$ being the \emph{feature domain}. We denote by $\GNof\Omega$ the set of all vertex-featured graphs with at most $N$ vertices and corresponding features in $\Omega$. Throughout the paper we use $\brc{}$ to denote multisets.
%

\ta{Say somewhere that our theory can straightforwardly accommodate edge features and explain how.}
%

\ta{Maybe say something about the graph isomorphism problem before introducing the WL test.}


\paragraph{Weisfeiler-Leman test}
%
The Weisfeiler-Leman (WL) graph isomorphism test is designed to determine whether two graphs are \emph{isomorphic}, meaning they are identical up to relabeling their nodes. The test either concludes that the graphs are non-isomorphic or returns an indeterminate outcome. Given $G=\br{V,E,X}$, the test follows the recursive formula
%
\begin{equation}\label{eqdef_wl}
\begin{split}
    c^{0}_{v} \eqdefx & \X_{v}, \quad v \in V, 
    %
    \\ c^{t}_{v} \eqdefx & \textup{Combine}\br{c^{t-1}_{v},\textup{Aggregate}\br{\setst{c^{t-1}_{u}}{u \in \N_{v}}}},
    \quad
    1 \leq t \leq T,
    %
    \\ c^{T}_G \eqdefx & \textup{Readout}\br{\brc{c^{T}_{v_{1}},\ldots,c^{T}_{v_{n}}}},
\end{split}
\end{equation}
%
where Aggregate and Readout are functions that injectively map multisets of vectors in Euclidean space into another Euclidean space, Combine is an injective function from one Euclidean space to another, and $\N_{v}$ denotes the neighborhood of the vertex $v$ in $G$. 

\begin{definition*}[WL graph equivalence]
Two vertex-featured graphs $G$ and $\tilde{G}$ are said to be \emph{WL-equivalent}, denoted by $G \wleq \tilde G$, if $c^T_G = c^T_{\tilde G}$ for all $T \geq 0$. Otherwise, they are said to be \emph{WL-separable} or \emph{WL-distinguishable}.
\end{definition*}
%

It is a known fact \citep{grohe2021logic,morris2023weisfeiler} that for $G,\tilde G \in \GNd$, if the equality $c^T_G = c^T_{\tilde G}$ is satisfied for $T=N$, then it is satisfied for all $T \geq 0$, and thus $G \wleq \tilde G$.

While the WL test can distinguish most pairs of non-isomorphic graphs, there exist examples of non-isomorphic graph pairs that WL cannot separate; see \citep{fail_example}.
%
Note that there exist higher-order versions of this test called $k$-WL, $k \geq 2$, but in this paper, we consider only the $1$-WL test, denoted by WL for brevity.


\paragraph{Functions on graphs}
%
A \emph{graph function} is a function $F:\GNd\to\RR^m$ that maps vertex-featured graphs into a Euclidean space. The output of a graph function should depend only on the structure of the input graph and its vertex features; specifically, it should be invariant to permuting the vertex indices. 

\begin{definition*}[WL separation]
    A graph function $F:\GNof\Omega\to\RR^m$ is said to be \emph{WL-separating} if for any pair $G,\tilde G \in \GNof\Omega$, $G \wlneq \tilde G$ implies $F\of{G} \neq F\of{\tilde G}$. If the converse also holds, then $F$ is said to be \emph{WL-equivalent}.
\end{definition*}

\paragraph{Graph embeddings}
Any WL-equivalent graph function can be regarded as injective when defined on the \emph{quotient space} of $\GNof\Omega$ with respect to WL equivalence. We denote that space by $\GNofWL\Omega$. Thus, such function provides an \emph{embedding} of $\GNofWL\Omega$ into the Euclidean space $\RR^m$.  

Euclidean embeddings are an essential tool in machine learning on non-Euclidean data, such as graphs. 
%These embeddings map inputs from the non-Euclidean data domain, in our case $\GNd$, into a Euclidean space. By doing so, 
They enable the application of multi-layer perceptrons (MLPs) and other standard machine learning techniques to the embedded space instead of the original non-Euclidean space.

Ideally, we would desire an embedding that produces different outputs for every pair of non-isomorphic graphs, namely an injective function from $\GNd$ to $\RR^m$. However, such an embedding would provide a solution to the graph isomorphism problem, to which no polynomial-time solution has been found to date. A reasonable compromise is an embedding that produces different outputs for pairs of graphs distinguishable by WL. %This motivates the following definition.



\paragraph{Message passing neural networks}
%
Message Passing Neural Networks (MPNNs) are the most common neural architectures designed to compute graph functions. They operate on a similar principle to the WL test, but with the purpose of performing predictions on graphs rather than determining if they are isomorphic. 

Their core mechanism is the message-passing procedure, which maintains a hidden feature for each vertex and iteratively updates it as a function of the neighbor's features.
%
This process is outlined as follows:
%
\begin{enumerate}
    \item \textbf{Initialization: } The hidden feature $\bh^{0}_v$ of each node is initialized by its input feature $\bx_v$.
    %
    \item \textbf{Message aggregation:} Each node $v\in V$ aggregates messages from its neighbors by
    %
    \begin{equation}
        m_v^{\br{t}} \eqdef \textup{Aggregate}\of{ \setst{ \phi\of{\bh^{\br{t-1}}_u} } {u \in \N_v} } 
    \end{equation}
    %
    with $\phi$ referred to as a \emph{message function}, and Aggregate is a multiset function.
    %
    \item \textbf{Update step:} Each node updates its own hidden feature according to its aggregated messages and its previous hidden feature:
    %
    \begin{equation}
        \bh^{\br{t}}_v \eqdef \psi\of{ m_v^{\br{t}}, \bh^{\br{t-1}}_v },
    \end{equation}
    %
    with $\psi$ referred to as an \emph{update function}.
    %
    \item \textbf{Readout:} After $T$ iterations of steps 2-3, a global graph-level feature $\bh_G$ is computed from the multiset of hidden features 
    $\setst{ h^{\br{T}}_v}{v\in V}$ 
    by a \emph{readout function}:
    \begin{equation*}
        \bh_G \eqdef \textup{Readout}\of{\setst{ h^{\br{T}}_v}{v\in V}}.
    \end{equation*}
\end{enumerate}
%
Numerous MPNNs were proposed in recent years \citep{gin,Gilmer2017NeuralMP}\ta{cite more examples}, with the main difference between them being the specific choices of the message, aggregation, update and readout functions. 


There is a close connection between MPNNs and the WL test, as it was shown by \citet{xu2018how,morris2019WL} that the expressive power of MPNNs is upper-bounded by that of WL. Namely, if the WL test does not distinguish between two graphs $G$, $\tilde G$, then any MPNN is guaranteed to produce the same output (as well as all intermediate values) on $G$ and $\tilde G$. Conversely, if all functions used in an MPNN are injective, then the graph function it computes is WL-equivalent.
\ta{Cite examples of WL-separating MPNNs}
Examples of such MPNNs are summation-based \cite{amir2023neural} etc.


\nd{suggestion: this should be after discussion of injectivity and why it is not enough. We therefore need a notion of a 'natural metric' on graphs. Here are two suggestions for such metrics...}


\paragraph{WL-equivalent metric for graphs}
%
While the WL test determines whether two graphs are WL-equivalent, in our setting, we consider graphs with continuous features. Therefore, a method that quantifies the \emph{extent} to which two graphs are not WL-equivalent would be a more appropriate tool. This motivates the following definition.
%
\begin{definition*}[WL-equivalent metric]
    A \emph{WL-equivalent metric on $\GNd$} is a function $\rho:\GNd \times \GNd \to \RR_{\geq 0}$ that satisfies the following conditions for all $G_1, G_2, G_3 \in \GNd$:
    \begin{subequations}
    \begin{align}        
        \rho\of{G_1, G_2} &\eqx \rho\of{G_2, G_1}
        & \quad &\textup{\emph{Symmetry} }
        %
        \\ \rho\of{G_1, G_3} &\leqx \rho\of{G_1, G_2} + \rho\of{G_2, G_3}
        & \quad &\textup{\emph{Triangle inequality} }
        %
        \\ \rho\of{G_1, G_2} &= 0 \Longleftrightarrow G_1 \wleq G_2.
        & \quad &\textup{\emph{WL equivalence} }
    \end{align}
    \end{subequations}
\end{definition*}
%
Note that strictly speaking, such $\rho$ is a \emph{pseudometric} on $\GNd$ rather than a metric, as it allows distinct graphs to have a distance of zero if they are WL-equivalent. However, for convenience, we will use the term \emph{metric} to denote a pseudometric.

%Note that the above definition depends on the parameter $N$.


\paragraph{Tree Mover's Distance}
%
We now describe a WL-equivalent metric for vertex-featured graphs proposed by \citet{TMD}. This metric, named the Tree Mover's Distance (TMD), is based on building computation trees that simulate the WL procedure, and calculating distances between sub-trees using optimal transport. With the full definition given in \ta{the next section / in the appendix}, the TMD, denoted by $\TMD[L]\of{G,\tilde G}$ depends on a depth parameter $L$. The authors proved that under some assumptions, for two graphs $G_1$, $G_2$, $\TMD[L+1]\of{G_1,G_2}>0$ if and only if $G_1$ and $G_2$ are distinguishable by $L$ iterations of WL.
%
% a tree distance between the WL computation trees parameterized by $L \in \NN$, which can be
% written recursively as the sum of the distance between tree roots $r$ and the distance
% between the sub-trees rooting at r’s children.
% By construction $TMD$ holds the following properties:
% \begin{enumerate}
%     \item $WL^{L}(\G) = WL^{L}(\H) \iff TMD^{L+1}(\G,\H) = 0$
%     \item Homogeneity with respect to multiplication of the node features by a scalar.
% \end{enumerate}
%
Note that this implies that for $L = N+1$, $\TMD[L]\of{\argdot,\argdot}$ is a WL-equivalent metric on $\GNd$.

%As mentioned above, the TMD is computed by recursion on computation trees that simulate the WL test. At the depth required for TMD to achieve WL-equivalence on $\GNd$, its worst-case computational complexity is $\mathcal{O}\of{N^5\log N}$. Our first main objective in this paper is to introduce a simpler metric, which can be computed by solving a linear program in $\mathcal{O}\of{\argdot}$ time \ta{complete this}. \nd{overkill. This is an extremely well known metric discussed in several very related work. See references I sent in the chat. We have the rather minor goal of extending it to features. This would seem straightforward to poeple familiar with the problem.}



\paragraph{Bi-Lipschitzness}
%
The main weakness of the notion of separation is that it does not provide any information about the \emph{quality} of the separation. Without further assumptions, a WL-separating function may map two input graphs that are far apart in a metric sense to outputs that are very close, or even numerically indistinguishable, in the output Euclidean space.
%
To produce numerically robust embeddings, one would expect an embedding function $\emb$ to map graphs that are far apart in the original space $\GNof\Omega$ to vectors that are similarly far apart in the embedding space, and vice versa. The most common mathematical property used to describe this behavior is \emph{bi-Lipschitzness}.
%
\begin{definition*}[bi-Lipschitz embedding]
    Let $\rho$ be a WL-equivalent metric on $\GNof\Omega$. An embedding $\emb:\GNof\Omega\to\RR^m$ is said to be \emph{bi-Lipschitz with respect to $\rho$ on $\GNof\Omega$} if there exist constants $0<c\leq C < \infty$ such that
    \begin{equation}\label{eqdef_bilip}
        c \cdot \rho\of{G_1,G_2}
        \leq \norm{\emb\of{G_1}-\emb\of{G_1}}
        \leq C \cdot \rho\of{G_1,G_2}
    \end{equation}
    for any $G_1, G_2 \in \GNof\Omega$.
    
    If $\emb$ satisfies just the left- or right-hand side of \cref{eqdef_bilip}, it is said to be \emph{lower-Lipschitz} or \emph{upper-Lipschitz}, respectively, with respect to $\rho$ on $\GNof\Omega$.
\end{definition*}
%
In \cref{eqdef_bilip} and throughout our paper, a norm $\norm{\argdot}$ without an order denotes the $\ell_2$ norm.

Bi-Lipschitzness essentially ensures that the embedding approximately preserves the original distances in the input space $\GNof\Omega$, with the ratio $\tfrac{C}{c}$ providing an upper bound on the distortion induced by the embedding, akin to the condition number of a matrix. A low-distortion embedding enables using metric-based learning methods such as nearest-neighbor search and data clustering in the embedding space instead of in the original space, where calculating pairwise metrics are typically significantly more computationally intensive.

Our second main objective is thus to develop an embedding for vertex-featured graphs that is bi-Lipschitz and can be computed efficiently in practice.


%Note that some embedding could be Bi-Lipschitz with respect to one metric but not with respect to another.

\paragraph{Oversmoothing and oversquashing}
aa\ta{Consider introducing these phenomena here and argue that the root underlying cause for the two of them is the lack of bi-Lipschitzness. Alternatively, introduce them in the next section, as an addition after stating the properties of our embedding.}
\nd{should I try to write something?}

To summarize our objectives, we want to (1) derive a WL-equivalent metric that is simple and easy to compute, and (2) develop a bi-Lipschitz embedding with respect to this metric that can be computed easily in practice.
%
We conjecture that such an embedding may help address the root cause of over-squashing. This will be confirmed by our experiments.



==> text_copy/subsec_related_works.tex <==
\subsection{Related Works}
\label{subsec_related_works}
%
\ta{Question to Nadav: Where is the optimal place to introduce oversquashing?}

\nd{all current related work has already been cited, and can be deleted. Things that are relevant are MPNN that used sorting or reference distributions, discussion of bilipschitzness for graphs in the literatures. Other mentions of bilipscitnzess. }

\ta{Move the two following paragraphs to the introduction or merge them into \cref{subsec_theoretical_background}. This subsection should contain methods that we have to cite but are not an integral part of the story.} \tared{Reminder}
%
\paragraph{graph isomorphism tests and GNNs}
As graph isomorphism is conjectured to be a hard problem, several graph isomorphism tests have been studied. The most famous is the WL test. In this test, the initial coloring of a node is its node feature, and the color is refined according to its color and neighbor's color. This test separates most graphs but not all \cite{fail_example}. A higher order of K-WL was introduced to separate more graphs, and it's known that (k+1)-WL can separate more graphs than K-WL but not all. \cite{Gilmer2017NeuralMP} showed that many methods fall under the message-passing neural networks framework. \cite{xu2018how,morris2019WL}, showed the 1-WL test bounds the expressiveness power of MPNNs. Thus, any two graphs 1-WL can't distinguish any MPNN will output the same embedding.
\paragraph{Graph Metrics}
Measuring distance between graphs is a topic in graph theory. A naive approach could be minimization over all permutations, but it's intractable. \cite{TMD} presented a distance equivalent to 1-WL and could be computed in a polynomial time.

